Generative models improve fairness of medical classifiers under distribution shifts

A ubiquitous challenge in machine learning is the problem of domain generalisation. This can exacerbate bias against groups or labels that are underrepresented in the datasets used for model development. Model bias can lead to unintended harms, especially in safety-critical applications like healthcare. Furthermore, the challenge is compounded by the difficulty of obtaining labelled data due to high cost or lack of readily available domain expertise. In our work, we show that learning realistic augmentations automatically from data is possible in a label-efficient manner using generative models. In particular, we leverage the higher abundance of unlabelled data to capture the underlying data distribution of different conditions and subgroups for an imaging modality. By conditioning generative models on appropriate labels, we can steer the distribution of synthetic examples according to specific requirements. We demonstrate that these learned augmentations can surpass heuristic ones by making models more robust and statistically fair in- and out-of-distribution. To evaluate the generality of our approach, we study 3 distinct medical imaging contexts of varying difficulty: (i) histopathology images from a publicly available generalisation benchmark, (ii) chest X-rays from publicly available clinical datasets, and (iii) dermatology images characterised by complex shifts and imaging conditions. Complementing real training samples with synthetic ones improves the robustness of models in all three medical tasks and increases fairness by improving the accuracy of diagnosis within underrepresented groups. This approach leads to stark improvements OOD across modalities: 7.7% prediction accuracy improvement in histopathology, 5.2% in chest radiology with 44.6% lower fairness gap and a striking 63.5% improvement in high-risk sensitivity for dermatology with a 7.5x reduction in fairness gap.

==> Learned Augmentations for medical images [arXiv]/background.tex <==
\section{Background}

Generative models, especially generative adversarial networks (GANs)~\citep{Goodfellow14}, have been employed by various studies to improve performance in different medical imaging tasks~\citep{Frid18,Ju21,Li19,Baur18,Rashid19}  and, in particular, for underrepresented conditions~\citep{Han20,Havaei21}. GAN-based augmentation techniques have not only been used for whole-image downstream tasks, but also for pixel-wise classification tasks~\citep{Zhao18,Uzunova20} with a more thorough review of those techniques provided by~\cite{Chen22}. Data obtained by exploring different latent image attributes through a generative  model has also been shown to improve adversarial robustness of image classifiers~\cite{Gowal_2020_CVPR}.

More recently, diffusion probabilistic models (DDPM)~\citep{Ho20, Nichol21,Nichol2021glide,Ho22} presented an outstanding performance in image generation tasks and have been probed for medical knowledge by~\cite{Kather22} in different medical domains. Other works extended diffusion models to 3D MR and CT images~\citep{khader2022medical} and demonstrated that they can be conditioned on text prompts for chest X-ray generation~\citep{chambon2022roentgen}. Given the ethical questions around the use of synthetic images in medicine and healthcare~\citep{Kather22,Chen21}, it is important to make a distinction between using generative models to \textit{augment} the original training dataset and \textit{replacing} real images with synthetic ones, especially in the absence of privacy guarantees. None of these works claims that the latter would be preferable, but rather come to the rescue when obtaining more abundant real data is either expensive or infeasible (e.g. in the case of rare conditions), even if this solution is not a panacea~\citep{Zhang22}. It is worth noting that while some studies view generative models as a means of replacing real data with `anonymized' synthetic data, we abstain from such claims as greater care needs to be taken in order to ensure that generative models are trained with privacy guarantees, as shown by~\cite{carlini2023extracting, Somepalli2022diffusion}.

\begin{figure}[t]
\includegraphics[clip, trim=0.0cm 2cm 0.0cm 1cm, width=\textwidth]{figures/generated_samples_all.pdf}
\caption{Samples generated by our conditional diffusion model for different imaging modalities.}
\label{fig:all_generated_modalities}
\end{figure}

%GAN-based approaches frame the problem of synthetic data generation as a minmax game, where the generator $\mathcal{G}$ aims to produce realistic samples that match the original data distribution, while a discriminator $\mathcal{D}$ aims to classify samples ashttps://braintex.goog/project/63976b845ee25900821849f4 real or fake, i.e. synthetic~\citep{Goodfellow14}. The better the generative model gets, the harder it becomes for the discriminator to distinguish between real and fake images. This behaviour can be achieved by adding an adversarial learning loss to the optimization objective. Depending on the application at hand, a generative model can be unconditional, i.e. $\mathcal{G}(z)$, with $z$ being a random latent vector that we feed to a decoder, or conditional on label information, i.e. $\mathcal{G}(z|c)$, with $c$ being a diagnostic or segmentation label. The decoder transforms the samples to the original image space, while the label(s) that the model is conditioned on can be used to `steer' the model along a particular axis, e.g. a sensitive attribute.

% Another class of GAN models rather focus on the issue of image translation and are more akin to CycleGAN~\citep{Zhu2017}, which was originally proposed to solve the image-to-image translation or style transfer task. These prove to be most useful in the presence of multiple modalities and can be trained in a supervised (if multimodal images are aligned) or unsupervised manner (if they are misaligned). As expected, this model class relies heavily on pixel-wise loss functions like cycle consistency, i.e. pixel-wise difference between the reconstructed and original images.

Recently, machine learning systems used for computer-aided diagnosis and clinical decision making have been scrutinized to understand their effect on sub-populations based on demographic or socioeconomic traits. Studies led by~\cite{Larrazabal20,Seyyed21,Puyol22} have investigated and identified discrepancies across groups based on gender / sex, age, race / ethnicity and insurance type (as a proxy of socioeconomic status), as well as their intersections.~\cite{Gianfrancesco18} performed a similar analysis for models operating on electronic health records. When evaluating machine learning systems in terms of certain fairness criteria, it is important to keep in mind that ensuring fairness in a source domain does not guarantee fairness in a different target domain under significant distribution shifts~\citep{Schrouff22}. Last but not least, there are multiple definitions of fairness in recent literature and different fairness metrics are often at odds with each other as noted by~\cite{Ricci22}. A more thorough review of related work is provided in~\autoref{sec:related_work}. In this work, we evaluate fairness both in- and out-of-distribution and aim to improve on fairness metrics without compromising top-level accuracy across all settings.

% \paragraph{Robustness to distribution shifts.}
% The goal of domain generalisation or robustness to distribution shifts is the ability of a predictor to perform well in an out-of-distribution setting. This can only be achieved by leveraging statistical invariances across training and test regimes. A few different techniques have been propose in the literature to address this challenge that include~\citep{Wiles21} \ira{Include citations for the following}:

% \begin{itemize}
%     \item \textit{Group Distributionally Robust Optimization (DRO)}, which perform Empirical Risk Minimization (ERM) while appropriately weighting domains with larger errors (so that they contribute a larger amount to the loss).
%     \item \textit{Inter-domain mixup}  that performs ERM on linear combinations of samples from random pair of domains and labels.
%     \item \textit{Domain-Adversarial Neural Networks (DANN)}, which employ an adversarial network that matches feature distributions across domains.
%     \item \textit{Invariant Risk Minimization} that learns a feature representation on top of which an optimizal linear classifier matches the same performance across domains given these representations.
% \end{itemize}

% \ira{Include a paragraph for DG techniques in health applications}



==> Learned Augmentations for medical images [arXiv]/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}



\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\lemmaref}[1]{Lemma~\ref{#1}}

\newcommand{\positive}{{\tt +}}
\newcommand{\negative}{{\tt -}}
\newcommand{\poscase}{\positive}
\newcommand{\negcase}{\negative}

\newcommand{\predvalidTrue}{{\tt valid}}
\newcommand{\predvalidFalse}{{\tt invalid}}

\newcommand{\consensuspositive}{{\tt consensus(+)}}
\newcommand{\consensusnegative}{{\tt consensus(-)}}
\newcommand{\leanpositive}{{\tt lean(+)}}
\newcommand{\leannegative}{{\tt lean(-)}}


\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\left[#1\right]}
%\newcommand{\E}[1]{\left\langle{#1}\right\rangle}

%\newcommand{\KL}{{\mathcal{KL}}}
\newcommand{\Wass}{{\mathcal{W}}}
\newcommand{\WassDiv}{{\mathcal{WD}}}
\newcommand{\dirac}{{\delta}}
\newcommand{\Dj}[1]{{\color{red} {#1}}}
\newcommand{\taylan}[1]{{\color{blue} {#1}}}
\newcommand{\sven}[1]{{\color{magenta} {#1}}}

\newcommand{\obs}{x}
\newcommand{\Obs}{X}
\newcommand{\lat}{z}
\newcommand{\Lat}{Z}
%alternative latent variable symbol
\newcommand{\altlat}{\zeta}
\newcommand{\altLat}{\mathcal{Z}}

\newcommand{\modeldeci}{d}
\newcommand{\predvalid}{v}
\newcommand{\humandeci}{h}
\newcommand{\systemdeci}{y}
\newcommand{\interdeci}{z}
\newcommand{\numexperts}{n}
\newcommand{\truedeci}{\systemdeci^{\text{true}}}


\newcommand{\dataset}{D}
\newcommand{\trainset}{D^{\text{train}}}
\newcommand{\tuneset}{D^{\text{tune}}}
\newcommand{\validset}{D^{\text{valid}}}
\newcommand{\thr}{\tau}
%\newcommand{\obs}{x}
\newcommand{\lbl}{y}
%\newcommand{\ind}[1]{\left[#1\right]}
\newcommand{\setoflabels}{\mathcal{Y}}
\newcommand{\setofobs}{\mathcal{X}}

\newcommand{\dispersion}{\epsilon}
\newcommand{\invtemperature}{\beta}
\newcommand{\params}{\theta}

\newcommand{\sigmoid}{\sigma}
\newcommand{\nnet}{\psi}

\newcommand{\istp}{\text{isTP}}
\newcommand{\istn}{\text{isTN}}
\newcommand{\isfp}{\text{isFP}}
\newcommand{\isfn}{\text{isFN}}

\newcommand{\tp}{\text{TP}}
\newcommand{\tn}{\text{TN}}
\newcommand{\fp}{\text{FP}}
\newcommand{\fn}{\text{FN}}

\newcommand{\auroc}{\text{AUROC}}
\newcommand{\sens}{\text{sensivity}}
\newcommand{\spec}{\text{specifity}}
\newcommand{\precision}{\text{precision}}
\newcommand{\recall}{\text{recall}}
\newcommand{\fone}{\text{F}_1}

% Entities
\newcommand{\ENTskincond}{skincond}
\newcommand{\ENTskintone}{skintone}
\newcommand{\ENTdatasource}{datasource}
\newcommand{\ENTgender}{gender}
\newcommand{\ENTage}{age}
\newcommand{\ENTriskbucket}{riskbucket}
\newcommand{\ENTcase}{case}
\newcommand{\ENTethnicity}{ethnicity}

\newcommand{\gumbeldist}{\mathcal{G}}
\newcommand{\expdist}{\mathcal{E}}
\newcommand{\rateparam}{\lambda}
\newcommand{\lograteparam}{\phi}
\newcommand{\meanparam}{\mu}

\newcommand{\rangeof}[1]{\{1,\dots,#1\}}
\newcommand{\uniformdist}{\mathcal{U}}

\newcommand{\MMATpredictions}{F}
\newcommand{\MMATgt}{Y}
\newcommand{\MMATmapping}{M}

\newcommand{\numclasses}{C}
\newcommand{\predset}{S}

% Plausibility score of case #1 and skin condition #2 
\newcommand{\plaus}[2]{\lambda^{#1}_{#2}}
% Total number of conditions
\newcommand{\numcond}{J}
\newcommand{\numreader}{R}

% The collection of choices of reader #1 for case #2 at rank #3
\newcommand{\block}[3]{B_{{#1}{#2}{#3}}}
\newcommand{\numblock}[2]{K_{{#1}{#2}}}

% The choice of reader #1 for case #2 at rank #3
\newcommand{\choice}[3]{\sigma_{{#1}{#2}{#3}}}
% The number of choices reader #1 has provided for case #2 
\newcommand{\numchoice}[2]{\mathbf{n}_{{#1}{#2}}}
% Latent arrival time for case #1 and condition #2 for reader #33  
\newcommand{\arrtime}[3]{\tau_{{#1}{#2}{#3}}}

\newcommand{\setofperms}{\mathcal{S}}

\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{thrm}[theorem]{Theorem}
\newtheorem{corro}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{dfn}[theorem]{Definition}

%\newcommand{\ind}[1]{\left[#1\right]}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eqdef}{\equiv}
%\newcommand{\E}[2]{\mathbb{E}_{#2}\left\{#1\right\}}
\newcommand{\E}[2]{\left\langle{#1}\right\rangle_{#2}}
\newcommand{\KL}{\mathcal{KL}}
\newcommand{\const}{\text{const.}}

\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Pmat}{\mathbf{P}}
\newcommand{\Pmatstage}[1]{\mathbf{P}^{(#1)}}
\newcommand{\pbase}{\mathbf{A}}
\newcommand{\cswap}[2]{\text{\tt cswap}(#1, #2)}

\newcommand{\pswap}[2]{\mathbf{E}_{#1,#2}}
\newcommand{\pbasestage}[1]{A^{(#1)}}
\newcommand{\pmat}{P}
\newcommand{\pmatij}{g}

\newcommand{\pmatq}{Q}
\newcommand{\pmatsort}{S}
\newcommand{\lamswap}{\lambda}
\newcommand{\rhoswap}{\rho}
\newcommand{\hardswap}{\rho}
\newcommand{\piswap}{\pi}



\newcommand{\pmatsoft}{\tilde{\mathbf{P}}}
\newcommand{\pmatsoftpinball}{\tilde{P}^{\text{pinball}}}
\newcommand{\pmatsoftstage}[1]{\tilde{P}^{(#1)}}
\newcommand{\Pmatsoft}{\tilde{\mathbf{P}}}
\newcommand{\setofPmat}{\mathbb{P}}
\newcommand{\Birkhoff}{\mathbb{B}}
\newcommand{\Birkhoffstage}[1]{\mathbb{B}^{(#1)}}
\newcommand{\Uppertri}{\mathbf{T}}
\newcommand{\uppertri}{T}
\newcommand{\Lowertri}{\mathbf{L}}
\newcommand{\lowertri}{L}
\newcommand{\ones}[1]{\mathbf{1}_{#1}}
\newcommand{\identity}[1]{\mathbf{I}_{#1}}
\newcommand{\Cost}{\mathbf{C}}
\newcommand{\cost}{C}
\newcommand{\costfun}{h}
\newcommand{\partitionfun}{Z}
\newcommand{\partitionfunhard}{\bar{Z}}
\newcommand{\objectivefun}{\Psi}
\newcommand{\dummyz}{z}

\newcommand{\dispersionalt}{\nu}
\newcommand{\x}{x}
\newcommand{\z}{z}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vxstage}[1]{\mathbf{x}^{(#1)}}
\newcommand{\xstage}[1]{{x}^{(#1)}}
\newcommand{\numstages}{K}
\newcommand{\stageidx}{k}

\newcommand{\y}{y}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vxsorted}{\tilde{\mathbf{x}}}
\newcommand{\snetedge}{e}
\newcommand{\snetEdgeset}{\mathcal{E}}
\newcommand{\snetedgeidx}{k}
\newcommand{\ki}{\snetedgeidx}
\newcommand{\snetnumedges}{K}
\newcommand{\K}{\snetnumedges}
\newcommand{\snet}{\mathcal{G}}

\newcommand{\testvec}{\mathbf{u}}
\newcommand{\testvecv}{\mathbf{v}}
\newcommand{\testmatu}{\mathbf{U}}
\newcommand{\testmatv}{\mathbf{V}}
\newcommand{\testveck}[1]{u_{#1}}
\newcommand{\expectation}{E}


\newcommand{\xsorted}{\tilde{x}}
\newcommand{\sort}{\text{\tt sort}}
\newcommand{\argsort}{\text{\tt argsort}}
\newcommand{\orderstat}{\text{\tt ostat}}
\newcommand{\ssort}{\text{\tt ssort}}
%\newcommand{\sigmoid}{\sigma}
\newcommand{\hrank}{\text{\tt rank}}
\newcommand{\srank}{\text{\tt srank}}
\newcommand{\hmax}{\text{\tt max}}
\newcommand{\hmin}{\text{\tt min}}
\newcommand{\hmedian}{\text{\tt median}}
\newcommand{\hquantile}{\text{\tt qtile}}
\newcommand{\quantiletau}{\tau}
\newcommand{\quantileenergy}{f}
\newcommand{\hargmin}{\text{\tt argmin}}
\newcommand{\hargmax}{\text{\tt argmax}}
\newcommand{\hismin}{\text{\tt ismin}}
\newcommand{\hismax}{\text{\tt ismax}}
\newcommand{\hzerooneloss}{\text{\tt zero-one-loss}}
%\newcommand{\crossent}{\text{\tt cross-entropy}}

\DeclareMathOperator{\relu}{relu}

\newcommand{\softmax}{\text{\tt softmax}}

\newcommand{\swapProb}{\text{\tt swapProbability}}


\newcommand{\htop}[1]{\text{\tt top}_{#1}}
\newcommand{\histop}[1]{\text{\tt istop}_{#1}}
\newcommand{\Ktop}{K}
\newcommand{\hattend}{\text{\tt attend}}
\newcommand{\basis}[1]{\mathbf{e}_{#1}}
\newcommand{\basisidx}{k}

\newcommand{\quantileparam}{\alpha}
\newcommand{\len}{n}
\newcommand{\lenm}{m}
\newcommand{\fun}{f}
\newcommand{\confmat}{C}
\newcommand{\ustat}{U}
\newcommand{\isgreater}{S}





\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
%\newcommand{\const}{\mbox{const}}
%\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
%\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
%\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
%\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
%\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
%\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\top}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
%\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

%\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
%\newcommand{\sign}{\mbox{sign}}
%\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
%\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
%\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> Learned Augmentations for medical images [arXiv]/discussion.tex <==
\section{Discussion}

In this work, we propose to use conditional generative models for improving robustness and fairness of machine learning systems applied to medical imaging. More specifically, we show that diffusion models can produce useful synthetic images in three different medical settings of varying difficulty, complexity and resolution: histopathology, radiology and dermatolgy. Our experimental evaluation provides extensive evidence that synthetic images can indeed improve statistical fairness, balanced accuracy and high risk sensitivity in a multi-class setting, while improving robustness of models both in- and out-of-distribution. In fact, we observe that generated data can be more beneficial out-of-distribution than in-distribution even in the absence of data from the target domain during training of the generative model (in the case of radiology). Generative models prove to be label efficient in both histopathology and dermatology settings, where we demonstrate that only a few labelled examples are sufficient for the diffusion models to capture the underlying data distribution well. This is particularly impactful in the medical setting, where data for particular conditions or demographic subgroups can be scarce or, even when available, acquiring expert labels can be expensive and time consuming. For the reader that is familiar with regularization techniques, we view diffusion models as another form of regularization, which can be combined with any other architecture or learning method improvements. 

Even though we do not make any assumptions when training the diffusion model, we find interesting dynamics when combining real and synthetic data. In certain settings, i.e., histopathology and radiology, we observe that we can rely purely on generated data and still outperform baselines trained with real labelled data (see~\ref{subsec:hist_label_eff}). In other settings, like dermatology, we observe that real data is more essential for training of the downstream discriminative model. We take a step further and analyze the impact of generated data and the mechanisms underlying the improvements in robustness and fairness that we report. Synthetic samples seem to better align distributions of different domains, while at the same time allowing models to learn more complex decision boundaries that reduce their reliance on spurious correlations. Finally, we highlight some practical benefits (highlighted in {\color{OliveGreen}green}) and discuss a number of potential risks (highlighted in {\color{purple}red}) and limitations (in {\color{BurntOrange}orange}) from relying on generated data.

\paragraph{\color{OliveGreen}Reusability of synthetic data.}
Beyond the analysis and utility of synthetic data for the particular tasks that we consider in this work, there are many other potential applications for which they can be useful. The same synthetic data can be used for data augmentation across different models and, potentially, tasks. For example, hand-crafted augmentations are often employed to introduce invariances and learn better representations in a self-supervised manner for a variety of downstream tasks.

\paragraph{\color{OliveGreen}Scalable approach.}
As we demonstrate in~\autoref{sec:toy_example}, if we have a perfect generative model then we can perform perfectly under the fair distribution.
Moreover, the better the generative model, the more our results should improve.
As a result, as generative modelling improves or as more data becomes available, results should improve accordingly.

\paragraph{\color{OliveGreen}Utility for leveraging private data sources.}
Combining this technique with privacy-preserving technologies holds a lot of promise in the medical field. One of the main reasons why transformative AI technologies have not yet demonstrated equivalent impact in the healthcare domain is due to regulations and limited data access. There is preliminary evidence that federated learning can be used to learn classification models from multiple institutions~\citep{Kaissis2021end} and if it were possible to generate private synthetic data, this synthetic data could be used for data augmentation along with a smaller, public dataset to improve performance.
This could have practical benefits when data sharing to protect personally identifiable information (PII) while achieving high quality performance. Such an approach would of course be associated with its own risks, some of which are discussed by~\cite{Cheng21}.

\paragraph{\color{purple}Overconfidence in the model.}
Even though we show that diffusion models can be particularly label efficient, this should not encourage practitioners to abandon their data and label acquisition efforts; nor does it imply that generated data can replace real data under any circumstances. What this research demonstrates is that, when labelled data and resources are limited, there are ways to make more of the available labelled and unlabelled data. There is also the potential that using generative models may lead to overconfidence in an AI system, because images look realistic to a non-expert.
Additional data collection will always be important, along with comprehensive analysis of the underlying data and its caveats.
Synthetic data from a generative model should {\em only} be used as a complement to additional data collection and accompanied by rigorous evaluation on real data, ideally outside the main source domain to understand generalization capabilities of the models. In other words, synthetic data is one solution to increase diversity, but not a substitution of efforts to increase data representation for underrepresented conditions and populations.

\paragraph{\color{purple}Bias in the training data.}
If the generative model is of poor quality or biased, then we may end up exacerbating problems of bias in the downstream model.
The generative model may be unable to generate images of a certain label and sensitive attribute. In other settings, the model may always generate a specific part of the distribution for a certain label and sensitive attribute instead of capturing the true image distribution.
The generative model may also create incorrect images of a given label and sensitive attribute, leading the classification model to make mistakes confidently in those regions. Therefore, it is particularly important that the evaluation data is unbiased.

\paragraph{\color{purple}Bias in the evaluation.}
The insights that we obtain by analyzing the model are only as good as our evaluation setup. If the evaluation datasets are not diverse enough, do not capture high-risk conditions well or are not representative of the population, then any conclusions we draw from these results will be limited. Therefore, care needs to be taken in order to report and understand what each of the evaluation setups is capturing. For example, as~\cite{varoquaux2022machine} highlight, clinician-level performance is often overstated without validating models out-of-distribution.

\paragraph{\color{BurntOrange}Categorical and unobserved attributes.} Sensitive attributes are not always observed or explicitly tracked and reported~\citep{Tomasev2021fairness}, often to protect people's privacy. At the same time, the way labels are assigned may have its own limitations. For example, using binary gender and sex attributes (or using the two interchangeably) does not represent people that identify as non-binary. Similarly, researchers have criticized the Fitzpatrick Skin Type because it is less accurate on shades of darker skin tones, which could cause models to misidentify or misrepresent people with darker skin. Similarly, there are other unobserved characteristics that can influence disease and are not accounted for in a visual image of skin, for example, like social determintants of health. One instance of this is how dermatitis on a person who lives in a communal setting could have a different differential diagnosis than dermatitis in a high on a high income individual. These are important considerations when relying on such attributes to condition learned augmentations or to perform fairness analyses.

\paragraph{\color{BurntOrange}Transparency when handling synthetic data.} Synthetic images should be handled with caution as they may perpetuate biases in the original training data. It is important to tag and identify when a synthetic image has been added to a database, especially when considering to reuse the dataset in a different setting or by different practitioners.


We see potential here for future work that improves fairness and out-of-distribution generalization by leveraging powerful generative models but without explicitly relying on pre-defined categorical labels. When we consider synthetic images as an option for addressing performance gaps across subgroups, the following challenges still need to be addressed: reducing memorization for rare attributes and conditions, providing privacy guarantees and accounting for unobserved characteristics.

==> Learned Augmentations for medical images [arXiv]/effect_synth_data.tex <==
\begin{document}
%\maketitle

\section{WORK IN PROGRESS!!! Investigating the effect of augmenting training data with synthetic samples}
Given the observed improvements on out-of-distribution generalization and fairness presented in the previous section, we now take a towards understanding \textit{why} synthetic data is being helpful. For that, we narrow our focus to the DermAssist dataset and compare models trained with synthetic data with different heuristic augmentation schemes, namely RandAugment REF*** and CT pipeline***. Post-hoc analysis isolating the effect of data augmentation: What happens to the features learned once we change the augmentation scheme? 

Previous work on out-of-distribution generalization REFs has pointed out that several factors can affect the performance of a model on samples from domains beyond the training data.  We analyse the considered models in light of distribution mismatch between all considered domains measure in the representation space induced by the learned models. We borrow tools from the out-of-distribution generalization literature: Distribution matching, 
alignment between distributions promotes better generalization REFS. Simplicity bias: 
Linear decision boundaries through the cost of relying on spurious correlations REFS. Previous work argues that: In case multiple features are equally predictive of labels on training data, neural networks will latch on the simpler ones. Simpler features might represent spurious correlations. This phenomena thus hurt out-of-distribution generalization of neural networks
Shah et al.,2020, Hermann and Lampinen, 2020, Nakkiran et al., 2019. 

Hypotheses: Is adding synthetic data helping the model to decrease the mismatch between in and out-of-distribution data? Is adding synthetic data enforcing the model to learn more complex (but still generalizable) features?

%\subsection{Procedure}

%\begin{algorithm}

%\end{algorithm}

\subsection{Feature alignment}
More specifically, we compute domain mismatches considering the space where decisions are performed, i.e. the output of the second-to-last layer of each model. We thus project each data point from the input space of size $\mathbb{R}^{64 \times 64}$ to a representation of size $\mathbb{R}^{6144}$. We compute 30 estimates of MMD between all pairs of domains using representations from the different models considering samples of size equal to 300. Mann-Whitney U test to the hypothesis that the data augmentation strategy has a significant effect on the pairwise MMD between domains. Models were under the same experimental conditions so that our analysis is capable of isolating the effect of data augmentation on the estimated pairwise distribution shifts. 

\begin{table}[h]
\begin{tabular}{ccccc}
\hline
\textbf{Domain 1}        & \textbf{Domain 2}       & \textbf{Synthetic data} & \textbf{RandAugment} & \textbf{CT} \\ \hline
\textbf{Enceladus Train} & \textbf{Narvi}          & 0.6279 $\pm$ 0.0823     & 0.4748 $\pm$ 0.0395  & 0.7778 $\pm$ 0.0930       \\
\textbf{Enceladus Train} & \textbf{Aegir}          & 0.0443 $\pm$ 0.0063     & 0.0332 $\pm$ 0.0065  & 0.0625 $\pm$ 0.0089       \\
\textbf{Enceladus Train} & \textbf{Enceladus Eval} & \textit{0.0121 $\pm$ 0.0047}   &  \textit{0.0128 $\pm$ 0.0054}  & 0.0209 $\pm$ 0.0079       \\
\textbf{Enceladus Train} & \textbf{Generated}      & 0.2472 $\pm$ 0.0190     & 0.1262 $\pm$ 0.0204  & 0.3580 $\pm$ 0.0524       \\
\textbf{Generated}       & \textbf{Narvi}          & 0.6992 $\pm$ 0.0706     & 0.4151 $\pm$ 0.0384  & 0.7682 $\pm$ 0.0915       \\
\textbf{Generated}       & \textbf{Aegir}          & 0.2794 $\pm$ 0.0187     & 0.1390 $\pm$ 0.0185  & 0.3766 $\pm$ 0.0444       \\
\textbf{Enceladus Eval}  & \textbf{Aegir}          & 0.0513 $\pm$ 0.0069     & 0.0413 $\pm$ 0.0073  & 0.0712 $\pm$ 0.0101       \\
\textbf{Enceladus Eval}  & \textbf{Narvi}          & 0.6107 $\pm$ 0.0731     & 0.4554 $\pm$ 0.0376  & 0.7596 $\pm$ 0.0859       \\
\textbf{Enceladus Eval}  & \textbf{Generated}      & 0.2374 $\pm$ 0.0175     & 0.1037 $\pm$ 0.0160  & 0.3052 $\pm$ 0.0472      \\
\textbf{Aegir}           & \textbf{Narvi}          & 0.5712 $\pm$ 0.0798     & 0.4216 $\pm$ 0.0402  & 0.7221 $\pm$ 0.0727       \\ \hline
\end{tabular}
\caption{}
\end{table}


\begin{itemize}
    \item Data augmentation has a significant effect on distribution alignment. Is synthetic data helping the model to better match different domains? Yes, in comparison to CT augmentations. Improvement on OOD performance suggests this is happening via learning better predictive features rather than capturing spurious correlations (as it seems to be happening for RA).
    \item Is generated data helping the model to better match different domains? Synthetic on top of the ct augmentations is helpful to decrease the overall discrepancy between domains.
    \item RandAugment vs Generated: rand augment yields representations that are more aligned, which can be helpful in case the model only relies on features that are stable across all domains, which doesn’t seem to be the case (c.f. to improved accuracy on Narvi, the most OOD domain wrt to Enceladus). Generated data, on the other hand, enforces the model to capture features that are helpful for predicting class labels on Narvi. 
    \item One hypothesis is that learning such features is conflicting with learning spurious correlations that were helpful for Enceladus and Aegir, therefore the decay in performance when adding generated data. 
    \item This can also be illustrated by the PCA analysis, where we found that adding RA or Gen aug enforced the model to learn more compressed (more generalizable in the sense that they overfit less to training data) representations. Generated data yielded “less compressed” representations and we hypothesized that this extra information was required to fit generated data.
    \item Is generated data enforcing the model to break spurious correlations that were mostly helpful for Enceladus and Aegir?
    \item Results might suggest that since CT+RA yielded more compressed representations (maybe the model found some correlations helpful for Enceladus and Aegir only) but worse performance on Narvi and generated data as well. Also, performance got worse when replacing RA by generated data.

\end{itemize}

\subsection{Simplicity bias}

We now investigate how complex* features learned by models trained with different augmentation schemes are. Complexity measure: number of principal components required to represent a percentage of the variance in the data.

It seems training with generated data enforces the model to ``spread out" data points from different domains in the learned representation space, yielding “less compressed” representations. We check for this hypothesis by comparing the number of principal components necessary to retain a given percentage of the variance in the data when performing PCA.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{./results/gen_data_analysis/PCA_5_seeds.png}
    \caption{. }
    \label{fig:pca_multiple_seeds}
\end{figure}

% Simplicity bias argument
\begin{itemize}
    \item Neural networks trained via SGD tend to find simpler models
    \item In case multiple features are equally predictive of labels on training data, neural networks will latch on the simpler ones
    \item Previous work further argues that simpler features might represent spurious correlations
    \item This phenomena thus hurt out-of-distribution generalization of neural networks
Shah et al., 2020, Hermann and Lampinen, 2020, Nakkiran et al., 2019
    \item Very recent work (ICLR submission), further argues that simplicity bias can also compromise fairness in case sub-group information is correlated with “hardness” of discrimination by a specific model
    \item We found synthetic data helps to decrease overall domain mismatch RA+CT < Gen+CT < CT only. Initially, hypothesized that domain generalization / adaptation theoretical results could explain OOD improvements with generated data
    \item However, OOD performance did not monotonically improved with distribution matching, especially in the case of Narvi
    \item PCA results indicate that RA+CT induces the model to learn features that occupy a smaller fraction of the embedding space 
    \item Given that, is it fair to argue that features learned by RA+CT are simpler? If so, perhaps we can further argue that synthetic augmentations help to mitigate simplicity bias. This happens because once we added generated data, simpler features that were useful in the case of RA+CT lose their predictive power, enforcing the model to make predictions based on more complex features. Then why did this effect not lead to overfitting? 
    \item Synthetic data promotes a better balance between feature complexity and out-of-distribution generalization
\end{itemize}



% Bibliography components
\bibliographystyle{abbrvnat}
\setlength{\bibsep}{5pt} 
\setlength{\bibhang}{0pt}
\bibliography{template_refs}


\end{document}

==> Learned Augmentations for medical images [arXiv]/introduction.tex <==
\section{Introduction}
The advent of machine learning (ML) in healthcare has led to many advances in various facets of care and in a wide range of applications~\citep{Esteva17,Ardila19,DeFauw18}.
For example, in dermatology, skin disease impacts at least 30\% of people worldwide \citep{Hay2014}, leading to 85 million doctor visits a year and a cost of \$75 billion~\citep{Lim17} in the US alone.
AI dermatological tools (e.g., \citealp{Esteva17,Liu20}) have the potential to allow patients to assess their conditions better and improve diagnostic accuracy \citep{Jain21}. Similarly, ML technologies have unlocked new capabilities in computational pathology which have the ability to handle the gigantic quantity of data created throughout the patient care lifecycle and improve classification, prediction, and prognostication of diseases~\citep{cui2021artificial}. These solutions are often motivated by the global shortage of expert clinicians, e.g., in the case of radiologists~\citep{rimmer2017radiologist}, and demonstrate that machine learning models can facilitate detection of conditions~\citep{rajpurkar2017chexnet}. Despite these rapid methodological developments and the promise of transformative impact in different areas of healthcare~\citep{liu2019comparison}, few of these approaches (if any) have achieved the ambitious goal of fostering clinical progress~\citep{varoquaux2022machine}. As~\cite{wilkinson2020time} highlight, only 24\% of published studies evaluate the performance of their proposed algorithms on external cohorts or compare this out-of-sample performance with that of clinical experts. Many studies do not validate the efficacy of algorithms in multiple settings and, the ones that do, often perform poorly when introduced to new environments not represented in the training data. 

Building a method that is robust across populations and subgroups, such that model performance does not degrade and benefits can be transferred when applied across groups, is a non-trivial task. This is due to data scarcity~\citep{castro2020causality}, challenges in the acquisition strategies of evaluation datasets, and the limitations of evaluation metrics. We list a number of key challenges here.
\textbf{(i)} \textit{Disease prevalence} may differ between demographic subgroups.
For example, melanoma is 26\% more likely to occur in white patients than black patients \citep{AmericanCancer}. Additionally, disease prevalence in the training data may not be reflective of the general population~\citep{Kaushal20}, which can be particularly problematic when due to disparities in access to healthcare~\citep{Khan21}.
However, over-reliance on such an attribute may lead to the model learning spurious correlations between those features and the diagnostic label or relying on `shortcuts'~\citep{Degrave2021,brown2022detecting}.
\textbf{(ii)} \textit{Data scarcity}. 
While we may be able to mitigate poor performance among subgroups or new domains by collecting more data, this can be infeasible due to disease scarcity, at odds with protecting patients privacy or just not sufficient for better and more generalizable solutions~\citep{varoquaux2022machine}.
\textbf{(iii)} \textit{Poor evaluation datasets}. It is vital to evaluate methods on datasets that reflect realistic shifts. For example, a population shift~\citep{Quinonero2008dataset} can lead to performance drop of the machine learning model across environments. In a realistic setting, we have limited control over the complexity of the shifts that arise, as shifts over multiple axes can occur simultaneously (e.g., both the acquisition protocol and the population at a new hospital may be different in a new geographic location). In healthcare, machine learning systems are often trained on data from a limited number of hospitals with the hope that they will generalise well to new unseen sites. However, if we focus on simpler synthetic settings, our conclusions may not generalise as demonstrated by \cite{Gulrajani20,Wiles21}.
\textbf{(iv)} \textit{High performance on overall accuracy metrics}, while important to track, \textit{may not always expose subtle problems}. For instance, it is possible to improve on top-1 accuracy by improving performance of the most prevalent class at the expense of performance on the minority classes. 

% Consequently, this work focuses on medical classification tasks, in which fairness under distribution shifts is a significant challenge, and validates how synthetic images (like the ones shown in~\autoref{fig:all_generated_modalities}) improve performance robustly under distribution shifts and positively impact statistical fairness across different axes.

Prior work has shown that a developed model may perform unexpectedly poorly on underrepresented populations or population subgroups in radiology~\citep{Larrazabal20,Seyyed21}, histopathology~\citep{yu2018classify} and dermatology~\citep{abbasi2020risk}. However, the issues of robustness to distribution shifts and statistical fairness have rarely been tackled together. In this work, we leverage generative models and potentially available unlabelled data to capture the underlying data distribution and \textit{augment} real samples when training diagnostic models across these three modalities. We show that combining synthetic and real data can lead to significant improvements in top-level performance, while closing the fairness gap with respect to different sensitive attributes under distribution shifts\footnote{We borrow the term \textit{sensitive attribute} from the fairness literature to describe demographic attributes we want the model to be fair against. All of the data used in this research was de-identified before DeepMind and Google gained access to it.}. Finally, we show that diffusion models are able to generate high quality images (see~\autoref{fig:all_generated_modalities}) across modalities and perform an in-depth analysis to shed light on the mechanisms that improve generalization capabilities of the downstream classifiers.

% First of all, machine learning algorithms often suffer from similar biases to the data they are trained on; this can occur when associations between the data and diagnoses are not reflective of the general population and can be problematic~\citep{Kaushal20}, particularly when this is due to disparities in access to healthcare~\citep{Khan21}. When the distribution of diagnoses in the training data is not reflecting that of the general population, the model encounters a label shift during deployment. In other settings, a population shift~\citep{Quinonero2008dataset} can lead to performance drop of the machine learning model across environments. This happens when a model is trained on a population that may be different from the population it is deployed on. In a clinical setting, a system is often trained on data from a limited number of hospitals with the hope that it will generalise well to new unseen sites. Finally, the training dataset may exhibit a long tail distribution over labels, sensitive attributes\footnote{We borrow the term \textit{sensitive attribute} from the fairness literature to describe demographic attributes we want the model to be fair against.} or intersections thereof. As a result, the developed model may perform unexpectedly poorly on underrepresented populations or population subgroups, which has been shown in radiology~\citep{Larrazabal20,Seyyed21}, histopathology~\citep{yu2018classify} and dermatology~\citep{abbasi2020risk}.




% ######### COMMENTS FROM OLDER VERSION #########

% A promising approach to improve performance in the context of data scarcity is to make use of generative models.
% This is a promising approach as (i) with a better generative model we expect further gains in performance and (ii) the generative and classification models do not need to be trained on the same data.
% For (ii), the generative model can be trained on held out, unlabelled and private data.
% Generative models have made great strides in creating photorealistic images \citep{Ramesh22,Karras18,Saharia22} and \cite{Levine20,Chen21} have demonstrated that there is a feasibility of combining generated data with real data to improve performance on using purely real data.
% However, these works stop short of demonstrating the utility of generated data in complex real world settings under challenging distribution shifts. In this work we devise a generative model that allows us to oversample underrepresented parts of the data distribution by sampling from an estimate of the prior. Intuitively, we use it as a data augmentation technique that, even though it ultimately does not recover parts of the distribution that are completely unobserved, it still complements parts where there are only few observed examples in the original training data. We show that this is a powerful augmentation technique in comparison to heuristic augmentations and other strong baselines, that allows us to improve on high-risk sensitivity and fairness across different sensitive attributes. 

% \section{Random thoughts from Olivia}

% If perfect generative model, could sample from missing parts of the distribution, fill in gaps, etc.
% Unrealistic.
% If imperfect, maybe still useful for distribution shift and fairness.
%  Why? Allows you to sample from an estimate of the prior. Can use, intuitively, as data augmentation but sample from under represented groups.
%  We explore using generated data in order to get a robust classifier. 
%  Explore on multiple modalities (\dermassist, etc.) and demonstrate we can consistently improve over baseline + improve fairness.
%  Iterative. 
% Ultimately we cannot recover parts of the distribution that are never observed, but we can oversample underrepresented parts.
% Intersectionality of generated images, i.e. can we assume that adopting the same ``style'' of one condition across skin tones is appropriate?

==> Learned Augmentations for medical images [arXiv]/maths.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softplus}{\zeta}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\lp}{\ensuremath{\ell_p}\xspace}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\maxmin}{max-or-min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\T}{^\textsf{T}}
\DeclareMathOperator*{\maximize}{max}
\DeclareMathOperator*{\minimize}{min}
\DeclareMathOperator{\proj}{proj}

%%%
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\Span{\textrm{Span}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\def\L{\mathcal{L}}




==> Learned Augmentations for medical images [arXiv]/methods.tex <==
\section{Method}

\begin{figure}[t]
    \centering
   \begin{overpic}[width=\linewidth,trim={0cm 5cm 0cm 0cm},clip]{figures/method.pdf}
   \put(6, 10){\small  $p_\texttt{train}(y)$}
   \put(29, 25){\small  $\hat{p}(\vx | y)$}
   \put(47, 25){\small  $\hat{p}(y)$}
   \put(78.5, 17.5){\small  $y_\texttt{pred} = f_{\tilde{\theta}}(\vx)$}
   \end{overpic}
    \caption{Overview of method. We use a labelled training set \datasettrain and an unlabelled training set to train a generative model $\hat{p}(\vx | y)$ from which we can sample data under a distribution $\hat{p}$. We combine generated, synthetic data with the labelled training set sampled from a distribution $p_\texttt{train}(y)$ in order to train the downstream classifier $f_{\tilde{\theta}}$. By combining synthetic and real data we aim to improve fairness and robustness under distribution shift. }
    \label{fig:method}
\end{figure}

We aim to leverage generated data to improve a downstream classifier's performance as motivated above.
We assume we have a dataset $D_\texttt{train} = \{ (\vx_i, c_i, \va_i)^N_{i=1} \}$  where $\vx_i, c_i$ is an image and label pair and $\va_i$ is a list of attributes about the datapoint.
In dermatology, the attributes may include sensitive attributes (such as gender, skin type, and age).
We have an additional dataset $D_\texttt{u} = \{ \hat{\vx_j}^M_{j=1} \}$ of unlabelled images which can be used as desired.
We have a generative model $\hat{p}_{\tilde{\theta}}$ trained with $D_\texttt{train}$ and $D_u$ (we make $\tilde{\theta}$ implicit in the following).
We drop the subscripts in the following for simplicity where obvious.

In order to achieve fairness, we assume we have some `fair' dataset $D_f = \{(\vx_i, y_i, \va_i)_{i=1}^F \}$ which are samples from the `fair' distribution $p_f$ over which we aim to minimize the expectation of the loss where $\vx_i, y_i$ is an image and label pair and $\va_i$ is a list of attributes about the datapoint (in dermatology, the attributes may include sensitive attributes such as gender, skin type, and age).
$Y$ is the number of labels and $|D_\cdot|$ denotes the size of the dataset.
\begin{equation}
    \min_\theta \sE_{D_f} \left( L(f_\theta(\vx), y, \va) \right)
    \label{eq:expectationfairness}
\end{equation}


We can decompose the data generating process into $p_f(\vx|\va, y)p_f(\va|y)p_f(y)$.
For example, we may have created $D_f$ by sampling uniformly over an attribute (such as gender) and labels.
We assume that the training dataset \datasettrain $\subset D_f$ is sampled from a distribution \ptrain where $p_\texttt{train}(x|\va, y) = p_f(\vx|\va, y)$
When $p_\texttt{train}(y, \va) \neq p_f(y, \va)$ then we have a  distribution shift between the training and fairness distribution (e.g.~the train distribution is more likely to generate images of a particular attribute than the fair distribution or combinations of label and attributes). 

We aim to combine the training dataset \datasettrain and synthetic data sampled from the generative model $\hat{p}$ in order to mimic most closely the fair distribution and improve fairness.
We construct a new dataset $\hat{D}_u$ according to a distribution $\hat{p}_u$ from these distributions using some probability parameter $\alpha$.
\begin{equation}
    (\vx, \va, y) \sim p' = 
    \begin{cases}
     (\vx, \va, y) \sim D_{\texttt{train}} \quad :  \alpha \\
    (\vx, \va, y), x \sim \hat{p}(\vx | y, \va), \va \sim \hat{p}(\va|y), y \sim \hat{p}(y) \quad : (1 - \alpha)  
    \end{cases}
\end{equation}
So instead of minimizing \autoref{eq:expectationfairness}, we minimize the following sum of expectations:
\begin{equation}
\label{eq:loss}
    \min_\theta \alpha \sE_{(\vx, \va, y) \sim D_{\texttt{train}}} \left( L(f_\theta(\vx), \va, y) \right) + (1 - \alpha) \sE_{(\vx, \va, y) \sim \hat{p}} \left( L(f_\theta(\vx), \va, y) \right) 
\end{equation}

The question is then how do we choose $\alpha$ and $\hat{p}(\va, y)$. To build an intuition of how to make these choices, we start with some toy setups. We assume that to minimise the loss in \autoref{eq:loss}, it is sufficient to minimize the KL divergence between the fair distribution $p_f$ and the combined distribution: $p'$.
For simplicity, we assume $p = p_\texttt{train} = p_f$ and that $\hat{p}(\va, y)$ is fixed.
The distribution shift arises from the finite dataset $D_\texttt{train}$ which may drift from $p$.
It is simple to extend these analyses to the more complex case where $p_\texttt{train} \neq p_f$.


\subsection{A Bernoulli distribution over a single variable.}
Here we assume there is a single variable $y$ we are trying to model that takes one of two values: $y \in \{0, 1\}$. 
Because $D_\texttt{train}$ is finite and consists $N$ samples, its distribution $t(y)$ may drift from $p$.
We also have a generative model $\hat{p}(y)$.
We assume the marginal distributions of these distributions are fixed.

We want to explore how we should combine $t(y)$ and $\hat{p}(y)$.
We can model this as saying we want to minimize the KL divergence between $p$ and $p'(y) = t(y) * (1 - \alpha) + \hat{p}(y) * \alpha$: $KL(p || p')$ where $\alpha$ is bounded by $[0, 1]$.
For example, if $p = \hat{p}$, then we should just sample from the generative model irrespective of $t$. Else, there is a trade off, and we can find the optimal $\alpha$ analytically or experimentally.

We next consider the more general setting.
We evaluate how using a generative model improves performance as we vary (1) the number of samples $N$ from $p$ when creating $D_\texttt{train}$; (2) $\hat{p}(y)$ and (3) $p(y)$.
We compare the distributions with and without generated data for a specific example in \autoref{fig:bernoulli_single}.
For a more thorough experiment, for each choice of values, we resample $t(y)$ 1000 times and experimentally find the optimal $\alpha$.
We plot the optimal $\alpha$ as we vary these values in \autoref{fig:bernoulli_comprehensive}.
As can be seen, using generated is generally helpful (by the fact that $\alpha > 1$).
We can also see various properties.
First, as $N$ increases (e.g.~there is less distribution shift between $D_\texttt{train}$ and $p$), using generated data becomes less helpful as $\alpha$ goes to $0$.
Second, generated data is most useful when its distribution is more similar to the true distribution $p$, but generated data is helpful even in the face of some distribution shift between $p$ and $\hat{p}$.


\begin{comment}
% OLD VERSION
The generative model may go wrong in multiple ways, which we discuss in turn and how this impacts these choices.

\paragraph{Generative model is perfect.} In this case, the generative model always generates images with $\hat{p}(\vx | \va, y) = p_f(\vx | \va, y)$.
Provided we know $p_f(\va, y)$, we can simply set $\alpha = 0$ and sample $(\va, y) \sim p_f(\va, y), \vx \sim \hat{p}(\vx | \va,  y)$.

\paragraph{The generative model perturbs the label and attribute distribution.}
In this case, when we generate images, we sometimes generate images with a label different from the conditioning one.
We model this as a perturbation on the sampled label:
$\hat{p}(x|y, \va) \equiv p(x|\bar{y}, \bar{\va})p(\bar{y}, \bar{\va}|y, \va)$.
where the conditioning label and attributes are $(y, \va)$ and the true label and attributes of $\vx$ under an oracle is ($\bar{y}, \bar{\va}$).
Here we may sample images that are from the true distribution but have the wrong label.
We assume that for all samples in $D_t$, a model will perform perfectly. 
In the case where $D_t = D_f$, synthetic data will not help and we should set $\alpha=1$.
Therefore, we can only improve performance on samples present in $D_f$ but missing in $D_\texttt{train}$.

\noindent {\em Case 1: $p_\texttt{train}(y, \va) \ll p_f(y, \va) \frac{|D_f|}{|D_\texttt{train}|}$ for some $(y, \va)$:} 
In this case there are parts of the train set with only a handful of samples, which leads to poor generalisation.
We can write this as that there are many samples $(\vx, y, \va) \in D_f$ for which $p_\texttt{train}(\vx | y, \va) \approx 0$.
On these samples, the model would have to generalise, and we assume it generalises with an accuracy $a_\texttt{train}(y, \va)$. \olivia{Could say this is random but I don't agree with that as you should generalise to some extent, depending on how much data you have.}

The question is under what conditions will adding imperfect synthetic data improve performance. If the generative model has a non zero chance of generating such samples, then it will classify it accurately with probability $\hat{p}(\bar{y}=y|y, \va)$.
We sample $S$ synthetic examples under $\hat{p}$ and assume they are all valid images in $D_f$.
\olivia{Could make more 'proofy' by decomposing the expectation.}
Then, if we assume infinite capacity of the model, the accuracy will be the weighted average of the accuracy on the samples in $D_\texttt{train}$ and the generated samples.
So for synthetic samples to be helpful, we need the following condition to hold:
\begin{align}
    \frac{|D_\texttt{train}|^{y, \va}a_\texttt{train}(y, \va) + S \hat{p}(\bar{y}=y|y, \va)}{|D_\texttt{train}|^{y, \va} + S} &> a_\texttt{train}(y, \va) \\
    |D_\texttt{train}|^{y, \va} &= p_\texttt{train}(y, \va) |D_\texttt{train}|
\end{align}
This holds when $\hat{p}(\bar{y}=y|y, \va) > a_\texttt{train}(y, \va)$.
If we assume that $a_\texttt{train}(y, \va)$ will be similar to the proportion of missing data, we can write this as 
$\hat{p}(\bar{y}=y|y, \va) > \min(1, \frac{|D_\texttt{train}|^{y, \va} }{|D_f| p_f(y, \va)})$.
This gives the first area where synthetic data is useful: (1) generating data for low density regions improves performance in that region over training with real data alone.

\noindent {\em Case 2: $p_\texttt{train}(y, \va) = 0$ for some $(y, \va)$:}
In this case, the train set does not cover the full distribution and includes missing regions for which there are no samples.
Intuitively, provided we have a model with infinite capacity and a non zero probability of generating samples from these low data regions which will be correctly labelled with better than chance, then using synthetic data will improve performance.
Provided $\hat{p}(\bar{y}=y, \bar{\va}=\va|y, \va) > \frac{1}{\prod_i A_i Y}$ (i.e., better than random guess) and $\hat{p}(\vx | y, \va) > 0$, we will improve performance (assuming a model with infinite capacity) by including samples with label and attribute $(y, \va)$.
\olivia{Proof by decomposing expectation into regions and saying that we will now do better on these regions so overall we will do better.}
This gives the second area where synthetic data is useful: (2) datapoints which do not exist in $D_\texttt{train}$ but are correctly generated and with a better than chance probability given the correct label by the generative model.
\olivia{Could just fold this into the above tbh.}

\paragraph{Discussion.} Under these three scenarios, we expect that using synthetic samples should improve on using real data alone. Moreover, we find the following areas where using synthetic data will help.
First, if the synthetic data is able to generate data in low density regions that is correct with a probability better than the accuracy of the model in that region using \datasettrain alone.
Second, if the generative model is able to generate samples that do not exist in \datasettrain and classify them correctly with an accuracy better than chance.
\end{comment}

\subsection{A Bernoulli distribution over a labelled and hidden variable.}
The above case does not take into account that we can resample the dataset and use the conditioning variable of the generative model to make $D_\texttt{train}$ and $\hat{p}$ more similar to $p$.
However, in reality while we may be able to resample on a labelled variable, there will be many hidden attributes that are important for fairness and generalization.
As we do not have labels for these hidden attributes, we {\em cannot} resample over them to make the distribution more similar to $p$.

To explore this in a simplistic setting, we proceed as follows.
We assume we have two variables $a, y$ where $y$ is the label and $a$ some hidden attribute
which we want to be fair over (and generalise over). Again, they follow a Bernoulli distribution: $a \in \{0, 1\}$ and $y \in \{0, 1\}$.

We condition on the label and we can sample arbitrarily according to the label but this gives us a distribution over attributes conditioned on the label, which is fixed.  We can sample arbitrarily to create $\bar{t}(y)$ and $\bar{p}(y)$ (provided $t(y), \hat{p}(y) > 0$) but $\bar{t}(a|y) = t(a|y)$ and $\bar{p}(a|y) = \hat{p}(a|y)$ is fixed.
Again, the question is how to optimally combine $t(y, a)$ and  $\hat{p}(y, a)$.
So now 
\begin{align}
p'(y, a) &= t(a|y)\bar{t}(y) + \hat{p}(a|y)\bar{p}(y) \\
\sum_y \bar{t}(y) + \bar{p}(y) &= 1 
\end{align}

And again we want to minimize the KL divergence between these two distributions, which can be factorized into the sum of the KL divergence between the marginal distribution over $a$ and conditional distribution over $y$.
\begin{align}
KL(p'(a, y) || p(a, y)) = KL(p'(y) || p(y)) + KL(p'(a|y) || p(a|y))
\end{align}
This is hard to solve analytically but we can find the optimal distributions of $\bar{t}, \bar{q}$ for a given set of distributions experimentally.

\subsection{A high dimensional Gaussian Mixture Model (GMM)}
Here we demonstrate that additional unlabelled data can improve classification performance in a very simple setting.
We assume that points come from an underlying GMM where each mixture in the GMM correspond to a different class.
This GMM can have varying number of dimensions (the number of features) and components (the number of classes).
We demonstrate that using a generative model fit to some number of unlabelled points in combination with the labelled points can lead to improved performance of a trained classifier.

Given some number of labelled and unlabelled points, the aim is to train a classifier that performs well on a held out validation set.
We do this by fitting a GMM to the unlabelled points and then using the labelled points to determine what class each mode belongs to by minimizing the classification error on the labelled points.
We then combine the labelled points and some number of points sampled from the GMM to form the training set. 
This is used to train the classifier, which is evaluated on the validation set.

We plot the evolution of the GMM being fit to the unlabelled points as the number of unlabelled points varies next to the true, underlying GMM in \autoref{fig:gmm_visualisation}.
We plot the fitted GMM for varying numbers of unlabelled points.
With only 500 unlabelled points, the fitted GMM matches pretty closely the true distribution.

We then run the full pipeline including the downstream classifier for varying numbers of labelled (sampled points), generated points, components, and dimensions.
We always use 10K unsupervised points.
To create the GMM, we randomly sample means from the range $[0, 1]$ for each dimension and we create a full covariance metric under a normal distribution with a scale of $0.1$.
We plot the results in \autoref{fig:gmm_results}. 
In these three cases, we can see that using additional generated data improves performance.
However, this does not always happen if (1) the classifier already performs near perfectly using the labelled data or (2) there is an insufficient number of points or the mixtures overlap so much that fitting the generative model gives a poor estimate of the underlying distribution.

\begin{figure}[t]
\centering
\begin{overpic}[width=0.24\textwidth]{gmm/gt.pdf}
\put(35,95){\tiny True Distribution}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_1.pdf}
\put(32,95){\tiny 5 Unlabelled Points}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_4.pdf}
\put(27,95){\tiny 500 Unlabelled Points}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_7.pdf}
\put(27,95){\tiny 5000 Unlabelled Points}
\end{overpic}
\caption{Visualising the fit GMM model for varying numbers of unlabelled points. Large points are labelled points, small points are unlabelled ones. Given only 500 unlabelled points, the fit distribution is similar to the true and with 5000 points, it matches the original. }
\label{fig:gmm_visualisation}
\end{figure}


\subsection{Discussion}
These toy experiments demonstrate that even in very simple settings, a generative model that complements in some way the data distribution can be used to create a new dataset that more closely mimics the underlying true distribution.
These two examples have shown in particular two scenarios where generative data can be especially helpful:
\begin{itemize}
    \item{\bf Missing regions.} Here the training data may not cover the full distribution. For example, if the training data has a label denoted by the random variable $y$ and attribute $a$ and there exists $y=y_c$, $a=a_c$ where there is no $x \in D_\texttt{train}$ such that $x \sim (y_c, a_c, ...)$.
    \item{\bf Low data regions.} Here there are only a few samples from parts of the distribution. If the generative model is able to capture this region then using additional samples from the generative model in this region should be helpful.
\end{itemize}

\section{Implementation}
\label{sec:implementation}

There are two main challenges. First, how to generate images with enough quality and diversity to be useful as additional synthetic data.
Second, how to combine real and synthetic data optimally for improved robustness and fairness.
We discuss these in turn.


\paragraph{The generator.}
We build on the diffusion model as popularized by \cite{Ho20}.
A diffusion model learns how to map images of gaussian noise to images from the distribution of training images.
Diffusion models have been leveraged to achieve state of the art, high quality results, with more diverse examples than with generative adversarial networks (GANs) \citep{Dhariwal21}.
The precise architecture we use is based on that of \cite{Dhariwal21} where we use a UNet with residual blocks and skip connections.

The architecture can be modified to allow for conditioning on auxiliary information \citep{Nichol21}, such as labels.
We use a one hot encoding of labels or labels and the sensitive attribute for conditioning.
When conditioning on both the label and sensitive attribute, we concatenate the one hot labels to form the final label.

\paragraph{Leveraging the unlabelled data.}
We can leverage ideas from classifier-free guidance to train a diffusion model with both labelled and unlabelled data.
Classifier-free guidance \citep{Ho21} trains both a conditional and unconditional diffusion model at the same time by randomly dropping some percentage of labels from the batch (by setting the label to $0$). 
At inference time, an image can be made more canonical by steering it away from the $0$-th label.
In our case, instead of randomly dropping labels, we treat the unlabelled data as dropped and set its label to the $0$-th label.
This allows us to train with both labelled and unlabelled data.
\olivia{Some insight here about how this modifies the sampling distribution.}

\paragraph{Super resolution?} Discuss how to work with larger image resolution sizes.

% \paragraph{Multiple instances?} Discuss how to generate multiple instances at once.

\paragraph{Combining real and synthetic data.}
The next step is to combine real and synthetic data.
Here there are two main considerations.
First, how to sample from the generative model and second how to trade-off between real and synthetic samples.
To sample from the generative model, we have to choose a distribution over the conditioning variable (the label or the label and auxiliary property).
We consider two distributions.
First, we can sample uniformly from the label or the joint distribution of label and auxiliary property.
However, this may harm overall performance.
Second, we can sample according to the label distribution in the training set but uniformly over the auxiliary property (if present).
This will increase diversity in the low data regions but not change the overall distribution of labels.
To trade-off between real and synthetic samples, we investigate combining batches of real and synthetic images with different ratios.
This effectively modifies the weight of the generative training in equation \ref{eq:finallikelihood}.


==> Learned Augmentations for medical images [arXiv]/results.tex <==
\section{Results}

\subsection{Overview of the proposed approach and experimental setting}

\begin{figure}[t]
% \includegraphics[clip, trim=0.1cm 2cm 0.1cm 3cm, width=\textwidth]{figures/method_overview.pdf}
\includegraphics[width=\textwidth]{figures/method_overview.pdf}
\caption{\textbf{Method overview.} In the proposed approach we first train a diffusion model on both labelled and unlabelled data (if available). In a general setting, unlabelled data may comprise of in- or out-of-distribution data (e.g., from an unseen hospital) for which we do not have expert labels. Subsequently, we sample synthetic images from the diffusion model according to particular specifications (e.g., an image of a female individual with pulmonary edema). Finally, we train a downstream classifier on a combination of the real labelled images and the synthetic images sampled from the diffusion model.}
\label{fig:overview}
\end{figure}

Our proposed approach (illustrated in~\autoref{fig:overview}) leverages generative models for learning augmentations of the data to improve robustness and fairness of medical machine learning models. It comprises three main steps: \textbf{(1)} We train a generative diffusion model given the available labelled and unlabelled data; we assume that labelled data is available only for a single, source domain, while additional unlabelled data can be from any domain (in- or out-of-distribution). We either condition the generative model only on the diagnostic label or on both the diagnostic label and a property (e.g., hospital id or sensitive attribute label). If high-resolution images are required ($>96 \times 96$ resolution), we further train an upsampling diffusion model in a similar manner. It is worth highlighting that both the low-resolution generative model and the upsampler are trained with the same conditioning vector (i.e. either with label or label \& property conditioning). \textbf{(2)} We sample from the generative model according to a fair sampling strategy. To do this, we sample uniformly from the sensitive attribute distribution, and preserve the original diagnostic label distribution in order to preserve the original disease prevalence. Sampling multiple times from the generative model allows us to obtain different augmentations for a given condition (and property) and increase the diversity of training samples for the downstream classifier. \textbf{(3)} We combine the synthetic images sampled from the generative model with the labelled data from the source domain and train a downstream classifier. We treat the mixing ratio of real to synthetic data as a hyperparameter that is application- and modality-specific. The classifier may have multiple heads and a shared backbone in the scenario where we require a separate prediction per diagnostic class.

\paragraph{Experimental protocol.}
We evaluate this approach using diffusion probabilistic models on different medical contexts and track top-level performance (e.g. accuracy) and fairness (when relevant) in- and out-of-distribution. The evaluation on out-of-distribution datasets is equivalent to developing a machine learning model on a certain population (e.g., from a particular hospital or geographic location) and testing its performance on a population from an unseen hospital or acquired under novel conditions. In all contexts, we consider the strongest and most relevant heuristic augmentations as a baseline. It is worth noting that these augmentations (heuristic or learned) can be combined with any alternative learning algorithm that aims to improve model generalization. For the sake of our experiments we use empirical risk minimization (ERM)~\citep{Vapnik1991principles}, as there exists no single method found to consistently outperform it under distribution shifts~\citep{Wiles21}. Even though our experiments and analysis focus on diffusion probabilistic models for generation, any conditional generative model that produces high-quality and diverse samples can be used.

\paragraph{Evaluation metrics.}
To measure the performance of the different baselines and the proposed method we use two sets of metrics: one set is more focused on accuracy (i.e. top-1 accuracy for histopathology, ROC-AUC for radiology and high-risk sensitivity for dermatology), while the second set is more geared towards fairness. The performance metrics vary depending on the classification task performed for each modality (i.e. binary vs. multi-class vs. multi-label) and consider label imbalance (tracking raw accuracy in a heavily imbalanced binary setting is not very insightful). For fairness we look at the performance gap (depending on the performance metric of interest) in the binary attribute setting and the difference between the worst and best subgroup performance for categorical attributes. For continuous sensitive attributes, like age, we discretize them into appropriate buckets (specified in~\autoref{sec:datasets}).

\subsection{Clinical Tasks and Datasets}

\subsubsection{Histopathology}

The first setting that we consider is histopathology. Different staining procedures followed by different hospitals lead to distribution shifts that can challenge a machine learning model that has only encountered images from a particular hospital. The CAMELYON17 challenge by~\cite{Bandi2018detection} aims to improve generalization capabilities of automated solutions and reduce the workload on pathologists that have to manually label those cases. The corresponding dataset contains whole-slide images from five different hospitals and the task is to predict whether the histological lymph node sections captured by the images contain cancerous cells, indicating breast cancer metastases. Two of the hospital datasets provided by the challenge are held-out for out-of-distribution evaluation and three are considered in-distribution, because they use similar staining procedures. We consider this as the simplest setting for our experiments, because there are no extreme prevalence or demographic shifts.  Additionally, the considered image resolution ($96 \times 96$) is smaller in comparison to the imaging modalities presented later, which allows generation directly at that resolution without requiring an upsampler. The labelled dataset contains $455,954$ images, while the unlabelled dataset contains $1.8$ million images from the three training hospitals; full statistics are given in \autoref{tab:camelyondatasetstatistics}.
The unlabelled dataset {\em does} contain the hospital identifier, but not the diagnostic label.

\begin{figure}[t]
    \centering
    \subfigure[In-distribution results]{ \includegraphics[width=0.62\linewidth]{results/camelyon/id_val_top1_accuracy_gap.pdf}}
    \subfigure[Out-of-distribution results]{ \includegraphics[clip, trim=0.0cm 6.2cm 0.0cm 0.0cm,width=0.35\linewidth]{results/camelyon/ood_test_top1_accuracy_all.pdf}}
    \caption{(a) In-distribution fairness gap (in percentage) between the best and worst performing hospital vs. overall prediction accuracy for the presence of breast cancer metastases in histopathology images. (b) Prediction accuracy (x-axis) on the validation and test hospitals when training the generative model on all in-distribution labelled examples (the y-axis corresponds to method index). Note that the validation set is used for model selection, given that its distribution is more similar to the training distribution. We compare the following methods: \textit{Baseline} model with no augmentations; \textit{Color augm} for a model that uses color augmentations; \textit{Label conditioning} and \textit{Label \& property conditioning} for our proposed approach of a generative model conditioned on the diagnostic label and both the diagnostic label and the hospital id, respectively; \textit{L cond + Color augm}, \textit{L \& P cond + Color augm} for applying color augmentations on the images generated with diffusion models. Combining color augmentation with synthetic data performs best across all settings.}
    \label{fig:camelyon_results}
\end{figure}

In order to understand the impact of the number of labelled examples on fairness and overall performance, we create different variants of the labelled training set, where we vary the number of samples from two of the three training hospitals (3 and 4). The number of labelled examples from one hospital remains constant. For each setting, we train a diffusion model using the labelled and unlabelled dataset (using only the diagnostic label whenever available in one case, and the diagnostic label together with the hospital id in the other case).
We, subsequently, sample synthetic samples from the diffusion model and train a downstream classifier that we evaluate on the held out in- and out-of-distribution datasets (results shown in~\autoref{fig:camelyon_results}).
We compare top-level classification accuracy and fairness gap, i.e. best-to-worst accuracy gap between the in-distribution hospitals to different baselines (more details about baselines are provided in~\autoref{subsec:baselines}).
We find that using synthetic data outperforms both baselines in-distribution in the less skewed (with 1000 labelled samples from hospitals 3, 4) and more skewed setting (with only 100 labelled samples) while closing the performance gap between hospitals. We obtain the best accuracy out-of-distribution when using all in-distribution labelled examples as shown in~\autoref{fig:camelyon_results}b (in the OOD setting there is one validation and one test hospital so we do not report a performance gap). 
We find that performing color augmentation on top of the generated samples generalizes best overall, leading to a $7.7\%$ absolute improvement over the baseline model on the test hospital.
This validates that indeed we can use synthetic data to better model the data distribution and outperform variants using real data alone. We also observe that this method is most effective in the low-data regime (i.e. more skewed setting in~\autoref{fig:camelyon_results}a). In~\autoref{fig:generated_image_clinical} we show some examples of healthy and abnormal histopathology images generated at $96 \times 96$ resolution.

\subsubsection{Chest Radiology}

\begin{figure}[t]
    \centering
    \subfigure[In-distribution condition co-occurrence]{ \includegraphics[width=0.49\linewidth]{results/chexpert/chexpert_train_joint_occurence.pdf}}
    \subfigure[Out-of-distribution condition co-occurrence]{ \includegraphics[width=0.49\linewidth]{results/chexpert/nih_eval_joint_occurence.pdf}}
    \caption{Heatmaps of normalized co-occurrence of conditions in the (a) CheXpert training and (b) the ChestX-ray14 evaluation datasets. For each condition on the row $r$ of the heatmap, the corresponding column $c$ indicates the ratio of all samples with condition $r$ that also have condition $c$. Note that more than two conditions can be present at once. We observe that in the training set it is much more common that more than one condition is present simultaneously.}
    \label{fig:cxr_condition_coexist}
\end{figure}

The second setting that we consider is radiology. We focus our analysis on two large public radiology datasets, CheXpert~\citep{Irvin2019chexpert} and ChestX-ray14 (US National Institutes of Health (NIH))~\citep{Wang2017chestx}. These datasets have been widely studied by the community~\citep{rajpurkar2017chexnet,Larrazabal20,Seyyed21} for model development and fairness analyses. For these datasets, demographic attributes like sex and age are publicly available, and classification is performed at a higher resolution, i.e. $224 \times 224$ like in~\cite{Azizi2022robust}. After training the generative model and classifier on 201,055 examples of chest X-rays from the CheXpert dataset, we evaluate on a held-out CheXpert test set (containing 13,332 images), which we consider in-distribution, and the test set of ChestX-ray14 (containing 17,723 images), which we consider out-of-distribution (OOD) due to demographic and acquisition shifts. We focus on five conditions for which labels exist in common between the two datasets\footnote{Note that the labelling procedures for the two datasets were defined and enacted separately, which likely increases the complexity of the task.}, i.e., \textit{atelectasis}, \textit{consolidation}, \textit{cardiomegaly}, \textit{pleural effusion} and \textit{pulmonary edema}, while each of these datasets contains more conditions (not necessarily overlapping), as well as examples with no findings, corresponding to healthy controls. In this setting the model backbone is shared across all conditions, while a separate (binary classification) head is trained for each condition, given that multiple conditions can be present at once.~\autoref{fig:cxr_condition_coexist} illustrates how often different conditions co-occur in the training and evaluation samples. It is apparent that capturing the characteristics of a single condition can be challenging given that in most cases they coexist with other conditions. One characteristic example is pleural effusion, which is included in the diagnosis of atelectasis, consolidation and edema in ~50\% of the cases. However, the scenario is slightly different for the OOD ChestX-ray14 dataset, where for most pairs of conditions the corresponding ratio is much lower. It is worth noting that the original CheXpert training set contains positive, negative, uncertain and unmentioned labels. The uncertain samples are not considered when learning the classification model, but they are used for training the diffusion model. The unmentioned label is considered a negative (i.e. the condition is not present) which yields a highly imbalanced dataset. Therefore, we report area under the receiver operating characteristic (ROC-AUC) curve in line with the CheXpert leaderboard, as raw accuracy is not very informative for such imbalanced settings.

% \ira{Plot joint distributions of conditions.} 
We observe that synthetic images improve the average AUC for the five conditions of interest in-distribution, but even more so out-of-distribution. Improvements are particularly striking for cardiomegaly, where the model trained purely with synthetic images improves AUC by $21.1\%$ (see~\autoref{fig:radiology_per_condition}). Overall, we observe an improvement of $5.2\%$ on average AUC OOD and a $44.6\%$ improvement in sex fairness gap (see~\autoref{fig:eval_auc_fairness_gap}). We show some examples of generated augmentations by the diffusion model for a model conditioned on the diagnostic label in~\autoref{fig:generated_image_clinical}. Higher resolution images are generated in comparison to histopathology with the use of a cascaded diffusion model that upsamples images generated at $64 \times 64$ resolution to $224 \times 224$.

\begin{figure}[t]
\includegraphics[width=\textwidth]{results/chexpert/cxr_224_auc_fairness_gap.pdf}
\caption{Comparison of average AUC vs. fairness (AUC) gap across different baselines for radiology. We report results in- (left column) and out-of-distribution (right column) on CheXpert and ChestX-ray14 datasets, respectively. We mark the baseline \textit{Pretrained on JFT} with black. \textit{Label conditioning} corresponds to the model that uses synthetic images from a diffusion model conditioned on only the diagnostic labels. We further compare to other strong contenders, i.e., a BiT-ResNet model pretrained on ImageNet-21K (\textit{Pretrained on IN-21K}), a model pretrained on JFT using RandAugment heuristic augmentations (\textit{RandAugment}), a model trained with RandAugment on top of standard ImageNet augmentations (\textit{RandAugment + IN Augms}) and a model trained with focal loss (\textit{Focal loss}). To ensure a fair comparison all methods are trained / finetuned for the same number of steps and with the same batch size. It is worth noting that for the fairness gap smaller values are preferable.}
\label{fig:eval_auc_fairness_gap}
\end{figure}

\subsubsection{Dermatology}

\begin{figure}[t]
\includegraphics[width=\textwidth]{figures/condition_distribution.pdf}
\caption{Condition distributions for in-distribution and out-of-distribution dermatology datasets. In-domain and OOD 2 distributions are much more similar in comparison to OOD 1. In particular, 3 out of 4 of the most prevalent conditions (i.e. acne, eczema and other) in the in-distribution dataset are also the most prevalent in OOD 2. However, there are only few examples of high-risk conditions like basal cell carcinoma and SCC/SCCIS, which are the two most prevalent conditions in OOD 1. We can see that overall the right-most dataset has a similar label distribution to the training dataset and, hence, is `less' out-of-distribution than the other one.}
\label{fig:eval_condition_stats}
\end{figure}

\begin{figure}[t]
\includegraphics[width=\textwidth]{results/64imagesize_1instance_v2/gender_64x1_high_risk_sensitivity_fairness_gap.pdf}
\caption{Comparison of high-risk sensitivity (for \texttt{basal cell carcinoma}, \texttt{melanoma}, \texttt{squamous cell carcinoma (SCC/SCCIS)} and \texttt{urticaria}) vs. fairness gap w.r.t. sex in dermatology across different baselines. We report results in- (left column) and out-of-distribution for OOD 1 (right column), as well as for the less skewed (top row) and more skewed (bottom row) setting. We mark the baseline \textit{Pretrained on JFT} with black. \textit{Label conditioning} and \textit{Label \& property conditioning} correspond to the models that use synthetic images sampled from a diffusion model conditioned on only the label, and the label and sensitive attribute, respectively. We further compare to other strong contenders, i.e., a BiT-ResNet model pretrained on ImageNet-21K (\textit{Pretrained on IN-21K}), a model pretrained on JFT using RandAugment heuristic augmentations (\textit{RandAugment}), a model trained with RandAugment on top of standard ImageNet augmentations (\textit{RandAugment + IN Augms}), a model trained on a resampled version of the training dataset that is more balanced w.r.t. to the sensitive attribute (\textit{Oversampling}) and a model trained with focal loss (\textit{Focal loss}). To ensure a fair comparison all methods are trained / finetuned for the same number of steps and with the same batch size. It is worth noting that for the fairness gap, smaller values are preferable.}
\label{fig:eval_high_risk_fairness}
\end{figure}

For the dermatology setting, we consider  a dermatology dataset of images at $256 \times 256$ resolution grouped into 27 labelled conditions ranging from low risk (e.g.~acne, verruca vulgaris) to high risk (e.g.~melanoma). Out of these conditions, four are considered to be high-risk: basal cell carcinoma, melanoma, squamous cell carcinoma (SCC/SCCIS) and urticaria. The imaging samples are often accompanied with metadata that include attributes, like biological sex, age, and skin tone.
Skin tone is labelled according to the Fitzpatrick scale\footnote{https://dermnetnz.org/topics/skin-phototype}, which gives rise to 6 categories (plus unknown). The ground truth labels for the condition are the result of aggregation of clinical assessments by multiple experts, who provide a list of top-3 conditions along with a confidence score (between 1-5). A weighted aggregate of these labels gives rise to soft labels that we use for training the diffusion and downstream classifier models.
For the purposes of our experiments we consider three datasets: the in-distribution dataset featuring 16,530 cases from a tele-dermatology dataset acquired from a population in the US (Hawaii and California); OOD 1 dataset featuring 6,639 images of clinical type focusing mostly on high-risk conditions from an Australian population, and OOD 2 featuring 3,900 tele-dermatology images acquired in Colombia.
These datasets are characterized by complex shifts with respect to each other as the label distribution, demographic distribution and capture process may all vary across them. To demonstrate the severity of the prevalence shift across locations, we visualise the distribution of conditions in the evaluation datasets in~\autoref{fig:eval_condition_stats}.
For training the downstream classifier, we use labelled samples from only one of these datasets (in-distribution), while we include unlabelled images from the other two distributions when training the diffusion model. We evaluate on a held-out slice of the in-distribution dataset and two out-of-distribution sets to investigate how well models generalize. We present results for OOD 2 only in Supplementary material~\ref{sec:supp_different_splits_derm}, as it has similar label distribution to the in-distribution dataset and is less challenging.

We explore whether the proposed approach can be used to {\em not only} improve out-of-distribution accuracy {\em but also} fairness over the different label predictions and attributes for the in-distribution distribution. Given that images considered for dermatology are high resolution, we train a cascaded diffusion model that upsamples images generated at $64 \times 64$ resolution to $256 \times 256$.
While the datasets are already imbalanced with respect to different labels and sensitive attributes, we also investigate how the performance varies as a dataset becomes more or less skewed along a single one of these axes. This allows us to better understand to what extent conditioning generative models on the axis of interest can help alleviate biases with regard to the corresponding attribute. For example, if our original dataset is skewed towards younger age groups, conditioning the generative model on age and (over)sampling from older ages can potentially help close the performance gap between younger and older populations\footnote{To study this aspect, we cannot rebalance our datasets as we have too few samples from the long tail of our distribution with regards to the label or sensitive attribute.}. We skew the training labelled dataset to make it progressively more biased (by removing instances from the least represented subgroups) and investigate how performance suffers as a result of the skewing.
For each sensitive attribute, we create new versions of the in-distribution dataset that are progressively more skewed to the high data regions. We show how the resulting training dataset are skewed with respect to each of the sensitive attributes in~\autoref{tab:sens_attr_splits_train}. 

In~\autoref{fig:eval_high_risk_fairness},  we illustrate for a single axis of interest how different methods compare with regards to sensitivity for the four high-risk conditions mentioned above and fairness. In the more skewed setting the training dataset contains a maximum of 100 samples from the underrepresented subgroup regardless of the underlying condition, while in the less skewed setting it contains maximum 1000 samples. We compare all methods in four different settings: in- and out-of-distribution as well as less and more skewed with respect to the sensitive attribute of interest, i.e. sex. We observe that in all settings, combining heuristic augmentations as in \textit{RandAugment + IN Augms} does improve the predictive performance across the board, but harms fairness of the model. Pretraining on a different dataset, on the other hand, has a negative impact on both performance and fairness (except for some performance improvement in the less skewed setting). Using \textit{RandAugment} alone is beneficial for high-risk sensitivity in-distribution, but not out-of-distribution, but it harms fairness in the OOD setting. \textit{Oversampling} slightly closes the fairness gap across the board while improving performance, as expected. The approaches that leverage synthetic data, \textit{Label conditioning} and \textit{Label \& property conditioning}, improve on high-risk sensitivity in-distribution without reducing fairness, while they yield a significant improvement in the OOD setting on both axes. In the more skewed setting, in particular, \textit{Label \& property conditioning} leads to $27.3\%$ better high-risk sensitivity compared to the baseline in-distribution and a striking $63.5\%$ OOD, while closing the fairness gap by $7.5\times$ OOD. It is worth noting that the underrepresented group in the training set and the ID evaluation set is over-represented in the OOD evaluation set. Our approach shows improvements in accuracy and fairness metrics with respect to different sensitive attributes, while being able to generalize these improvements out-of-distribution as shown in~\ref{sec:supp_different_splits_derm}.

\begin{comment}
\paragraph{Results at resolution $64\times64$.}
For each sensitive attribute and distribution shift, we run all baselines with five random seeds.
We then train a diffusion model at $64\times64$ using the labelled and unlabelled data for that specific shift and combine synthetic and real data.
We consider conditioning either only on the label or on the label and sensitive attribute.
We plot both the accuracy and balanced accuracy on the in distribution datasets (\enceladus) and out-of-distribution datasets (\aegir, \narvi) in \autoref{fig:accuracy_results}.
We plot the fairness metrics in \autoref{fig:fairness_results} and the high risk sensitivity in \autoref{fig:risk_results}.

First, we discuss results on the accuracy metrics. Across all distribution shifts and all datasets, using generated data either improves or maintains the accuracy metrics on \dermassist.
In particular, generated data seems to help most on the out-of-distribution dataset \narvi and on the balanced accuracy metric.
We can see that using heuristic augmentation is also helpful here, in particular RandAugment consistently improves over the baseline.
The other methods (oversampling and focal loss) give minimal improvements.

Next, we investigate results on the fairness metrics in \autoref{fig:fairness_results}.
Here, we see that using heuristic augmentation leads to no consistent improvement over the baseline.
However, for sex, skintone, and age, our approach of using generated data consistently improves on or maintains the performance of the baseline model.
We find that this is true {\em even on out-of-distribution datasets} such as \narvi and \aegir.
This is impressive as \cite{Schrouff22} demonstrated that improving fairness on in-distribution datasets does not guarantee performance improvements on out-of-distribution datasets.
(Note that there are no skin tone labels for \narvi and \aegir, so for skintone we only report results on \enceladus.)

Finally, we investigate how using synthetic data impacts high risk sensitivity in \autoref{fig:risk_results}.
In diagnostics, it is imperative to not miss someone with a high risk condition.
As a result, we investigate whether using synthetic data negatively or positively impacts the model's ability to correctly identify images of a high risk condition.
Of the $27$ classes, four of them are identified as high risk conditions: \texttt{Basal Cell Carcinoma}, \texttt{Melanoma}, \texttt{SCC/SCCIS}, and \texttt{Urticaria}.
By adding additional data we want to improve (or at least not harm) high risk sensitivity.
We investigate the high risk sensitivity on both the training dataset (\enceladus) and the two out-of-distribution datasets (\aegir, \narvi).
We find that across distribution shifts and datasets, using the additional synthetic data either maintains or improves high risk sensitivity, most notably on \narvi (one of the out-of-distribution datasets).
Moreover, synthetic data is consistently similar or better than heuristic augmentation on this metric.

We find that on dermassist, using synthetic has a host of benefits. 
While it can to some extent improve balanced accuracy while maintaining overall accuracy, additional synthetic data can improve fairness metrics both in and out-of-distribution and high risk sensitivity for both in and out-of-distribution datasets.
This demonstrates that using synthetic data as augmentation has promise for improving fairness and the diagnosis of high risk conditions.

\olivia{Do we need a sweep over different $\gamma$ for the focal loss?} \olivia{Should check some of the larger error bars and ensure all seeds are being evaluated.}
\end{comment}

\begin{figure}
    \centering
    \subfigure[Cyst, melanolytic nevus, seborrheic dermatitis]{\includegraphics[clip, trim=3cm 0cm 3cm 0cm,width=0.49\linewidth]{results/dermatology/dermatology_gen_a_clipped.pdf}}
    \subfigure[Folliculitis, hidradenitis, alopecia areata]{ \includegraphics[clip, trim=3cm 0cm 3cm 0cm,width=0.49\linewidth]{results/dermatology/dermatology_gen_b_clipped.pdf}}
    \caption{Generated images in dermatology setting; each row of images corresponds to a different condition.}
    \label{fig:generated_image_natural}
\end{figure}

\subsection{In depth analysis for dermatology}
In this section our analysis focuses on the last modality of dermatology.

\subsubsection*{Generated images are diverse}
First, we show images generated at $256 \times 256$ resolution for this challenging, natural setting and a number of dermatological conditions in~\autoref{fig:generated_image_natural}. We highlight that our conditional generative model does capture the characteristics well for multiple, diverse conditions, even for cases that are more scarce in the dataset, such as \texttt{seborrheic dermatitis}, \texttt{alopecia areata} and \texttt{hidradenitis}. 

\subsubsection*{Generated images are realistic}
We further evaluate how realistic the generated images are as determined by expert dermatologists to validate that these images do contain properties of the disease used for conditioning.
We note that the synthetic images do not need to be perfect, as we are interested in downstream performance.
However, being able to generate realistic images validates that the generative model is capturing relevant features of the conditions.
To evaluate this, we ask dermatologists to rate a total of 488 synthetic images each, evenly sampled from the four most common classes (\texttt{eczema}, \texttt{psoriasis}, \texttt{acne}, \texttt{SK/ISK}) and four high risk classes (\texttt{melanoma}, \texttt{basal cell carcinoma}, \texttt{urticaria}, \texttt{SCC/SCCIS}). 
They are tasked to first determine if the image is of a sufficient quality to provide a diagnosis.
They are then asked to provide up to three diagnoses from over 20,000 common conditions with an associated confidence score (out of 5, where 5 is most confident).
These 20,000 conditions are mapped to the 27 classes we use in this paper (where one class, \texttt{other}, encompasses all conditions not represented in the other 26 classes).
We report mean and standard deviation for all metrics across the three raters.
$50.0 \pm 12.6\%$ of those images were found to be of a sufficient quality for diagnosis, while dermatologists had an average confidence of $4.13 \pm 0.43$ out of $5$ for their top diagnosis.
They had a top-1 accuracy of $56.0 \pm 11.9$\% on the generated images and a top-3 accuracy of $67.7 \pm 12.5$\%. We compare these numbers to a set of real images of the same eight conditions considered above (for the images considered, the majority of raters consider diagnosis of this disease as most prevalent in the image). Amongst 101 board certified dermatologists rating 789 real images in total\footnote{For this analysis, if an image has been rated by $N$ dermatologists, we consider a single rater's accuracy with respect to the aggregated diagnosis of the remaining $N-1$ raters.}, we found that their top-1 accuracy was $54.0 \pm 21.1$\% and top-3 accuracy $67.1 \pm 22.7$\%; slightly higher performance in terms of top-1 (63\%) and top-3 accuracy (75\%) was shown in \citep{Liu20} across a more diverse set of dermatological conditions.
This demonstrates that, when diagnosable as per experts' evaluation, synthetic images are indeed representative of the condition they are expected to capture; similarly so to the real images. Even though not all generated images are diagnosable, this can be the case for real samples as well, given that images used to train the generative model do not necessarily include the body part or view that best reflects the condition.

% We analyse generated images more thoroughly to understand how they help medical models become more robust and fair. We have the following hypotheses that we want to test:

% \begin{itemize}
% \item Synthetic images are more canonical examples of the condition.
% \item Synthetic images are diverse with respect to the body part and the severity of the condition.
% \item Synthetic images allow models to align distributions better and lead to better generalization.
% \item Synthetic images reduce spurious correlations, i.e. information that is domain-specific.
% \item Synthetic images allow accurate classification of high-risk conditions across demographic groups.
% \end{itemize}

\subsubsection*{Generated images are canonical}
We hypothesize that the reason why models become more robust to prevalence shifts is due to synthetic images being more canonical examples of the conditions. To understand how canonical ground truth images for a particular condition are, we investigate cases with high degree of concordance in raters' assessments and compare those to synthetic images for the same condition. More specifically, we threshold the aggregated ground truth values to filter the images within the training data that experts were most confident about presenting a condition. The aggregation function operates as follows: assume we have a set of 4 conditions $\{A, B, C, D\}$; if rater $R_1$ provides the following sequence of (\texttt{condition}, \texttt{confidence}) diagnosis tuples: $\{(A, 4), (B, 3)\}$ and rater $R_2$ provides $\{(A, 3), (D, 4)\}$, then we obtain the following soft labels $\{0.5, 0.167, 0, 0.333\}$ (after weighting each condition with the inverse of its rank for each labeller, summing across labellers and normalising their scores to 1).
% unnormalised labels \{1.5, 0.5, 0, 1.0\}$ 
If we look for instances for which there is consensus amongst raters and high-confidence that a condition is present we can threshold the corresponding soft label for that condition with a strict threshold, e.g. $t=0.9$. In our example, this doesn't hold for any of the 4 conditions, but if we lowered the threshold to 0.5, then it would hold for condition $A$.
In~\autoref{fig:canonical_image_diversity} we show an example for melanoma. For this particular diagnostic class we are able to generate multiple synthetic instances of the condition, while we recovered only 5 images (out of $>15,000$) that clinicians rated with high confidence, i.e. $t_{\textrm{melanoma}}=0.9$. The nearest neighbours from the training dataset identified based on $\ell^2$-norm are also shown in~\autoref{fig:canonical_image_diversity}.
% The images with high confidence in the ground truth across all datasets show that generated images are more diverse with respect to the body parts they are capturing. 
\begin{comment}
We further ran a small-scale experiment with clinical experts to understand whether generated images are diagnosable and representative of the condition.
\end{comment}
% Quantitative.

\begin{figure}[t]
\includegraphics[clip, trim=0.0cm 4cm 0.0cm 1cm, width=\textwidth]{figures/image_diversity.pdf}
\caption{(\textit{Left}) The diffusion model can produce an infinite amount of synthetic images for a particular condition that is inherently more scarce (we have fewer than 50 samples of melanoma in our training dataset). (\textit{Middle}) The images that experts have identified with melanoma with high confidence (a combination of individual's confidence in diagnosis and expert consensus). (\textit{Right}) The nearest neighbours from the training samples identified for each of the synthetic images based on $\ell^2$-norm in pixel space.}
\label{fig:canonical_image_diversity}
\end{figure}


\subsubsection*{Generated images align feature distributions better}
Previous work on out-of-distribution generalization \citep{Ben2010theory, Muandet2013domain, Albuquerque2019generalizing} has pointed out that several factors can affect the performance of a model on samples from domains beyond the training data. In this analysis, we investigate the models trained with our proposed learned augmentations in terms of changes in distribution alignment between all pairs of distributions measured via the Maximum Mean Discrepancy (MMD)~\citep{Gretton2012kernel}, as previous work has empirically shown that approaches based on learning features that decrease MMD estimates yield improved out-of-distribution generalization~\citep{Li2018domain}. We compute domain mismatches considering the space where decisions are performed, i.e., the output of the penultimate layer of each model. We thus project each data point from the input space to a representation. We find that learned augmentations yield on average 18.6\% lower MMD in comparison to heuristic augmentations (for more details refer to~\ref{sec:supp_different_splits_derm}) which leads to the following conclusions: (i) Data augmentation has a significant effect on distribution alignment. Improvement on OOD performance suggests this is happening via learning better predictive features rather than capturing spurious correlations. (ii) Generated data helps the model to better match different domains by attenuating the overall discrepancy between domains. (iii) Given the minor decline in performance when adding generated data in the less skewed setting as shown in~\autoref{fig:eval_high_risk_fairness}, these findings suggest that learning such features might conflict with learning spurious correlations that were helpful for in-distribution performance.

\subsubsection*{Synthetic images reduce spurious correlations}

To further compare the effect of different augmentation schemes on the features learned by the downstream classifier, we investigate the representation space occupied by all considered datasets, including samples obtained from the generative model. In practice, we project $N$ randomly sampled instances from each dataset to the feature space learned by each model and apply the Principal Component Analysis algorithm~\citep{abdi2010principal}. We then extract the number of principal components required to represent different fractions of the variance across all instances projected to the feature spaces induced by models obtained with heuristic and learned augmentations.
% In~\autoref{fig:pca_analysis}, we show the average number of components required to retain $\{0.60, 0.70, 0.80, 0.90, 0.95\}$ of the variance of the projected data obtained across five different model initializations for both learned and heuristic augmentations. 
We observe that for a fixed dataset, features from models trained with synthetic data require 5.4\% fewer principal components to retain 90\% of the variance in latent feature space (results for different fractions are provided in~\autoref{fig:pca_analysis}). This indicates that using synthetic data induces more compressed representations in comparison to augmenting the training data in a heuristic manner. Considering this finding in the context of the results in~\autoref{tab:mmd_domains}, we posit the observed effect is due to domain-specific information being attenuated in the feature space learned by models trained with synthetic data. This suggests that our proposed approach is capable of reducing model's reliance upon correlations between inputs and labels that do not generalize out-of-distribution.


==> Learned Augmentations for medical images [arXiv]/theoretical_motivation.tex <==
\section{Old write ups for theoretical motivation.}
\subsection{Theoretical Motivation 1}

To motivate why using generated samples should improve a classifier, we take inspiration from \cite{Lasserre07}. 
We first summarize their setup before describing how we utilise their framework.
We first assume we have a generative model which is specified as the product of the prior over classes $p(c|\pi)$ with the class conditional density $p(\vx|c,\lambda)$, where $\vtheta = \{ \pi, \lambda \}$.
This can be rewritten in terms of the likelihood $L_G(\vtheta)$.

\begin{align}
    p(\vx, c | \vtheta) = p(c | \pi) p(\vx | c, \lambda) \\
    L_G(\vtheta) = p(\rmX, \rmC, \vtheta) = p(\vtheta) \prod_{n=1}^N p(x_n, c_n | \vtheta)
\end{align}

However, as explained by \cite{Minka05} and \cite{Lasserre07}, we cannot simply use discriminative training, as that changes the model itself, not just the training method.
Instead \cite{Lasserre07} and \cite{Minka05} construct a new likelihood function $q$ that introduces a new set of parameters $\Tilde{\theta}$.
\begin{align}
    q(\vx, \vc| \vtheta, \Tilde{\vtheta}) &= p(\vc|\vx, \vtheta)p(\vx| \tilde{\vtheta}) \\
    p(\vx|\Tilde{\vtheta}) &= \sum_{\vc'}p(\vx, \vc'|\Tilde{\vtheta})
\end{align}

\cite{Lasserre07} then assume that the prior over parameters $p(\vtheta, \Tilde{\vtheta})$ factorizes:
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) = p(\vtheta)p(\Tilde{\vtheta})
\end{align}

This gives the following function to be maximised:
\begin{align}
    q(\rmX, \rmC, \vtheta, \Tilde{\vtheta}) &= p(\vtheta, \tilde{\vtheta}) \prod_{n=1}^{N} p(c_n | x_n, \vtheta)p(x_n|\Tilde{\vtheta}) \\
    &= \left[ p(\vtheta) \prod_{n=1}^{N} p(c_n| x_n, \vtheta) \right]  \left[ p(\Tilde{\vtheta}) \prod_{n=1}^{N} p(x_n | \Tilde{\vtheta}) \right]
\end{align}

\paragraph{An equality prior.}
If the parameters are independent then this is simply discriminative training.
The question is how to construct the prior over $\vtheta, \Tilde{\vtheta}$ when the parameters $\vtheta, \Tilde{\vtheta}$ are not independent.
\cite{Lasserre07} consider an equality prior.
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) = p(\vtheta)\delta(\vtheta - \Tilde{\vtheta})
\end{align}
If $\Tilde{\vtheta} = \vtheta$ then we can see that the joint distribution of $q$ simplifies to the original generative model.
This can be loosened by considering priors from a laplace distribution to give a smooth transition between pure discriminative/generative training.
Which set up is optimal depends whether the data is truly from the generative model.
If it is, then the hard constraint is preferable, allowing for the use of the additional data.
If it is not, then we can still improve on discriminative training depending on how the generative model is constructed and the additional, unlabelled data improves model performance. This requires experimental investigation in practice.

\paragraph{Forcing consistency.}
In our case, it is not simple to impose a constraint directly on the model parameters, as the models are trained separately with different model parameters. Instead, we aim to achieve the coupling of the generative and discriminative models by imposing a consistency constraint in the prior.
Now, instead of in \cite{Lasserre07}, we do not consider an equality prior but instead a prior that predictions must be consistent between the two models. 

 If the generator generates an image, label pair $(x'_k, c'_k)$ with image $x'_k$ and label $c'_k$ then the discriminative model should predict that sample to have the same label.
We have the following where $\rmX'$ denotes the $N_s$ sampled images and $\rmC'$ the sampled classes and we assume $\vtheta, \Tilde{\vtheta}$ are independent variables. \olivia{I don't think this is right: should be integrating over $x'_k, {c'_k}$ which would give a sum. All this should be checked by Taylan.}:
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC' | \vtheta, \Tilde{\vtheta})} \\
     &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC' |
    \vtheta) p(\rmX', \rmC' | \Tilde{\vtheta})} \\
     &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC') p(\rmX', \rmC' | \Tilde{\vtheta})} \\
    p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC') &= p(\vtheta, \Tilde{\vtheta} | \rmX', \rmC') p(\rmX', \rmC') \\
    &= p(\vtheta |\rmX', \rmC') p(\Tilde{\vtheta} | \rmX', \rmC') p(\rmX', \rmC') \\
    &= \frac{p(\vtheta)p(\rmC' | \rmX', \vtheta)}{p(\rmC' | \rmX')} p(\rmX', \rmC' | \Tilde{\vtheta}) p(\Tilde{\vtheta}) \\
    p(\vtheta, \Tilde{\vtheta}) &= \frac{p(\vtheta)p(\rmC' | \rmX', \vtheta)}{p(\rmC' | \rmX')^2 p(\rmX')} p(\Tilde{\vtheta}) \\
\end{align}

Now we assume these samples are independent to get a new joint distribution:
\begin{align}
    q(\rmX, \rmC, \vtheta, \Tilde{\vtheta}) = \left[ \prod_{n=1}^{S} \frac{p(c'_n|x'_n, \vtheta)}{p(c'_n|x'_n)^2 p(x'_n)} \right] \left[ p(\vtheta) \prod_{n=1}^{N} p(c_n| x_n, \vtheta) \right]  \left[ p(\Tilde{\vtheta}) \prod_{n=1}^{N} p(x_n | \Tilde{\vtheta}) \right]
    \label{eq:finallikelihood}
\end{align}

\paragraph{Special case: the generative model subsumes the training set.}
If the generative model subsumes the training set and is perfect than $p(c'_n | x'_n) = 1, p(x'_n) = 1$ and we can see that optimizing the discriminative model over the generated samples is sufficient to optimize it over the real samples. 

If it is not, then optimizing the discriminative model over the generated samples amounts to having a regularizer with a weight $\lambda$ that is controlled by the coefficient $\frac{1}{\prod_{n=1}^{N_s} p(c'_n|x'_n)^2 p(x'_n)}$. 
As this quantity is unknown, we can sweep over this value experimentally (from $1$ to $\infty$) to find the optimal trade off for the discriminative model between generated and real examples.

==> effect_synth_data.tex <==
\begin{document}
%\maketitle

\section{WORK IN PROGRESS!!! Investigating the effect of augmenting training data with synthetic samples}
Given the observed improvements on out-of-distribution generalization and fairness presented in the previous section, we now take a towards understanding \textit{why} synthetic data is being helpful. For that, we narrow our focus to the DermAssist dataset and compare models trained with synthetic data with different heuristic augmentation schemes, namely RandAugment REF*** and CT pipeline***. Post-hoc analysis isolating the effect of data augmentation: What happens to the features learned once we change the augmentation scheme? 

Previous work on out-of-distribution generalization REFs has pointed out that several factors can affect the performance of a model on samples from domains beyond the training data.  We analyse the considered models in light of distribution mismatch between all considered domains measure in the representation space induced by the learned models. We borrow tools from the out-of-distribution generalization literature: Distribution matching, 
alignment between distributions promotes better generalization REFS. Simplicity bias: 
Linear decision boundaries through the cost of relying on spurious correlations REFS. Previous work argues that: In case multiple features are equally predictive of labels on training data, neural networks will latch on the simpler ones. Simpler features might represent spurious correlations. This phenomena thus hurt out-of-distribution generalization of neural networks
Shah et al.,2020, Hermann and Lampinen, 2020, Nakkiran et al., 2019. 

Hypotheses: Is adding synthetic data helping the model to decrease the mismatch between in and out-of-distribution data? Is adding synthetic data enforcing the model to learn more complex (but still generalizable) features?

%\subsection{Procedure}

%\begin{algorithm}

%\end{algorithm}

\subsection{Feature alignment}
More specifically, we compute domain mismatches considering the space where decisions are performed, i.e. the output of the second-to-last layer of each model. We thus project each data point from the input space of size $\mathbb{R}^{64 \times 64}$ to a representation of size $\mathbb{R}^{6144}$. We compute 30 estimates of MMD between all pairs of domains using representations from the different models considering samples of size equal to 300. Mann-Whitney U test to the hypothesis that the data augmentation strategy has a significant effect on the pairwise MMD between domains. Models were under the same experimental conditions so that our analysis is capable of isolating the effect of data augmentation on the estimated pairwise distribution shifts. 

\begin{table}[h]
\begin{tabular}{ccccc}
\hline
\textbf{Domain 1}        & \textbf{Domain 2}       & \textbf{Synthetic data} & \textbf{RandAugment} & \textbf{CT} \\ \hline
\textbf{Enceladus Train} & \textbf{Narvi}          & 0.6279 $\pm$ 0.0823     & 0.4748 $\pm$ 0.0395  & 0.7778 $\pm$ 0.0930       \\
\textbf{Enceladus Train} & \textbf{Aegir}          & 0.0443 $\pm$ 0.0063     & 0.0332 $\pm$ 0.0065  & 0.0625 $\pm$ 0.0089       \\
\textbf{Enceladus Train} & \textbf{Enceladus Eval} & \textit{0.0121 $\pm$ 0.0047}   &  \textit{0.0128 $\pm$ 0.0054}  & 0.0209 $\pm$ 0.0079       \\
\textbf{Enceladus Train} & \textbf{Generated}      & 0.2472 $\pm$ 0.0190     & 0.1262 $\pm$ 0.0204  & 0.3580 $\pm$ 0.0524       \\
\textbf{Generated}       & \textbf{Narvi}          & 0.6992 $\pm$ 0.0706     & 0.4151 $\pm$ 0.0384  & 0.7682 $\pm$ 0.0915       \\
\textbf{Generated}       & \textbf{Aegir}          & 0.2794 $\pm$ 0.0187     & 0.1390 $\pm$ 0.0185  & 0.3766 $\pm$ 0.0444       \\
\textbf{Enceladus Eval}  & \textbf{Aegir}          & 0.0513 $\pm$ 0.0069     & 0.0413 $\pm$ 0.0073  & 0.0712 $\pm$ 0.0101       \\
\textbf{Enceladus Eval}  & \textbf{Narvi}          & 0.6107 $\pm$ 0.0731     & 0.4554 $\pm$ 0.0376  & 0.7596 $\pm$ 0.0859       \\
\textbf{Enceladus Eval}  & \textbf{Generated}      & 0.2374 $\pm$ 0.0175     & 0.1037 $\pm$ 0.0160  & 0.3052 $\pm$ 0.0472      \\
\textbf{Aegir}           & \textbf{Narvi}          & 0.5712 $\pm$ 0.0798     & 0.4216 $\pm$ 0.0402  & 0.7221 $\pm$ 0.0727       \\ \hline
\end{tabular}
\caption{}
\end{table}


\begin{itemize}
    \item Data augmentation has a significant effect on distribution alignment. Is synthetic data helping the model to better match different domains? Yes, in comparison to CT augmentations. Improvement on OOD performance suggests this is happening via learning better predictive features rather than capturing spurious correlations (as it seems to be happening for RA).
    \item Is generated data helping the model to better match different domains? Synthetic on top of the ct augmentations is helpful to decrease the overall discrepancy between domains.
    \item RandAugment vs Generated: rand augment yields representations that are more aligned, which can be helpful in case the model only relies on features that are stable across all domains, which doesn’t seem to be the case (c.f. to improved accuracy on Narvi, the most OOD domain wrt to Enceladus). Generated data, on the other hand, enforces the model to capture features that are helpful for predicting class labels on Narvi. 
    \item One hypothesis is that learning such features is conflicting with learning spurious correlations that were helpful for Enceladus and Aegir, therefore the decay in performance when adding generated data. 
    \item This can also be illustrated by the PCA analysis, where we found that adding RA or Gen aug enforced the model to learn more compressed (more generalizable in the sense that they overfit less to training data) representations. Generated data yielded “less compressed” representations and we hypothesized that this extra information was required to fit generated data.
    \item Is generated data enforcing the model to break spurious correlations that were mostly helpful for Enceladus and Aegir?
    \item Results might suggest that since CT+RA yielded more compressed representations (maybe the model found some correlations helpful for Enceladus and Aegir only) but worse performance on Narvi and generated data as well. Also, performance got worse when replacing RA by generated data.

\end{itemize}

\subsection{Simplicity bias}

We now investigate how complex* features learned by models trained with different augmentation schemes are. Complexity measure: number of principal components required to represent a percentage of the variance in the data.

It seems training with generated data enforces the model to ``spread out" data points from different domains in the learned representation space, yielding “less compressed” representations. We check for this hypothesis by comparing the number of principal components necessary to retain a given percentage of the variance in the data when performing PCA.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{./results/gen_data_analysis/PCA_5_seeds.png}
    \caption{. }
    \label{fig:pca_multiple_seeds}
\end{figure}

% Simplicity bias argument
\begin{itemize}
    \item Neural networks trained via SGD tend to find simpler models
    \item In case multiple features are equally predictive of labels on training data, neural networks will latch on the simpler ones
    \item Previous work further argues that simpler features might represent spurious correlations
    \item This phenomena thus hurt out-of-distribution generalization of neural networks
Shah et al., 2020, Hermann and Lampinen, 2020, Nakkiran et al., 2019
    \item Very recent work (ICLR submission), further argues that simplicity bias can also compromise fairness in case sub-group information is correlated with “hardness” of discrimination by a specific model
    \item We found synthetic data helps to decrease overall domain mismatch RA+CT < Gen+CT < CT only. Initially, hypothesized that domain generalization / adaptation theoretical results could explain OOD improvements with generated data
    \item However, OOD performance did not monotonically improved with distribution matching, especially in the case of Narvi
    \item PCA results indicate that RA+CT induces the model to learn features that occupy a smaller fraction of the embedding space 
    \item Given that, is it fair to argue that features learned by RA+CT are simpler? If so, perhaps we can further argue that synthetic augmentations help to mitigate simplicity bias. This happens because once we added generated data, simpler features that were useful in the case of RA+CT lose their predictive power, enforcing the model to make predictions based on more complex features. Then why did this effect not lead to overfitting? 
    \item Synthetic data promotes a better balance between feature complexity and out-of-distribution generalization
\end{itemize}



% Bibliography components
\bibliographystyle{abbrvnat}
\setlength{\bibsep}{5pt} 
\setlength{\bibhang}{0pt}
\bibliography{template_refs}


\end{document}

==> methods.tex <==
\section{Method}

\begin{figure}[t]
    \centering
   \begin{overpic}[width=\linewidth,trim={0cm 5cm 0cm 0cm},clip]{figures/method.pdf}
   \put(6, 10){\small  $p_\texttt{train}(y)$}
   \put(29, 25){\small  $\hat{p}(\vx | y)$}
   \put(47, 25){\small  $\hat{p}(y)$}
   \put(78.5, 17.5){\small  $y_\texttt{pred} = f_{\tilde{\theta}}(\vx)$}
   \end{overpic}
    \caption{Overview of method. We use a labelled training set \datasettrain and an unlabelled training set to train a generative model $\hat{p}(\vx | y)$ from which we can sample data under a distribution $\hat{p}$. We combine generated, synthetic data with the labelled training set sampled from a distribution $p_\texttt{train}(y)$ in order to train the downstream classifier $f_{\tilde{\theta}}$. By combining synthetic and real data we aim to improve fairness and robustness under distribution shift. }
    \label{fig:method}
\end{figure}

We aim to leverage generated data to improve a downstream classifier's performance as motivated above.
We assume we have a dataset $D_\texttt{train} = \{ (\vx_i, c_i, \va_i)^N_{i=1} \}$  where $\vx_i, c_i$ is an image and label pair and $\va_i$ is a list of attributes about the datapoint.
In dermatology, the attributes may include sensitive attributes (such as gender, skin type, and age).
We have an additional dataset $D_\texttt{u} = \{ \hat{\vx_j}^M_{j=1} \}$ of unlabelled images which can be used as desired.
We have a generative model $\hat{p}_{\tilde{\theta}}$ trained with $D_\texttt{train}$ and $D_u$ (we make $\tilde{\theta}$ implicit in the following).
We drop the subscripts in the following for simplicity where obvious.

In order to achieve fairness, we assume we have some `fair' dataset $D_f = \{(\vx_i, y_i, \va_i)_{i=1}^F \}$ which are samples from the `fair' distribution $p_f$ over which we aim to minimize the expectation of the loss where $\vx_i, y_i$ is an image and label pair and $\va_i$ is a list of attributes about the datapoint (in dermatology, the attributes may include sensitive attributes such as gender, skin type, and age).
$Y$ is the number of labels and $|D_\cdot|$ denotes the size of the dataset.
\begin{equation}
    \min_\theta \sE_{D_f} \left( L(f_\theta(\vx), y, \va) \right)
    \label{eq:expectationfairness}
\end{equation}


We can decompose the data generating process into $p_f(\vx|\va, y)p_f(\va|y)p_f(y)$.
For example, we may have created $D_f$ by sampling uniformly over an attribute (such as gender) and labels.
We assume that the training dataset \datasettrain $\subset D_f$ is sampled from a distribution \ptrain where $p_\texttt{train}(x|\va, y) = p_f(\vx|\va, y)$
When $p_\texttt{train}(y, \va) \neq p_f(y, \va)$ then we have a  distribution shift between the training and fairness distribution (e.g.~the train distribution is more likely to generate images of a particular attribute than the fair distribution or combinations of label and attributes). 

We aim to combine the training dataset \datasettrain and synthetic data sampled from the generative model $\hat{p}$ in order to mimic most closely the fair distribution and improve fairness.
We construct a new dataset $\hat{D}_u$ according to a distribution $\hat{p}_u$ from these distributions using some probability parameter $\alpha$.
\begin{equation}
    (\vx, \va, y) \sim p' = 
    \begin{cases}
     (\vx, \va, y) \sim D_{\texttt{train}} \quad :  \alpha \\
    (\vx, \va, y), x \sim \hat{p}(\vx | y, \va), \va \sim \hat{p}(\va|y), y \sim \hat{p}(y) \quad : (1 - \alpha)  
    \end{cases}
\end{equation}
So instead of minimizing \autoref{eq:expectationfairness}, we minimize the following sum of expectations:
\begin{equation}
\label{eq:loss}
    \min_\theta \alpha \sE_{(\vx, \va, y) \sim D_{\texttt{train}}} \left( L(f_\theta(\vx), \va, y) \right) + (1 - \alpha) \sE_{(\vx, \va, y) \sim \hat{p}} \left( L(f_\theta(\vx), \va, y) \right) 
\end{equation}

The question is then how do we choose $\alpha$ and $\hat{p}(\va, y)$. To build an intuition of how to make these choices, we start with some toy setups. We assume that to minimise the loss in \autoref{eq:loss}, it is sufficient to minimize the KL divergence between the fair distribution $p_f$ and the combined distribution: $p'$.
For simplicity, we assume $p = p_\texttt{train} = p_f$ and that $\hat{p}(\va, y)$ is fixed.
The distribution shift arises from the finite dataset $D_\texttt{train}$ which may drift from $p$.
It is simple to extend these analyses to the more complex case where $p_\texttt{train} \neq p_f$.


\subsection{A Bernoulli distribution over a single variable.}
Here we assume there is a single variable $y$ we are trying to model that takes one of two values: $y \in \{0, 1\}$. 
Because $D_\texttt{train}$ is finite and consists $N$ samples, its distribution $t(y)$ may drift from $p$.
We also have a generative model $\hat{p}(y)$.
We assume the marginal distributions of these distributions are fixed.

We want to explore how we should combine $t(y)$ and $\hat{p}(y)$.
We can model this as saying we want to minimize the KL divergence between $p$ and $p'(y) = t(y) * (1 - \alpha) + \hat{p}(y) * \alpha$: $KL(p || p')$ where $\alpha$ is bounded by $[0, 1]$.
For example, if $p = \hat{p}$, then we should just sample from the generative model irrespective of $t$. Else, there is a trade off, and we can find the optimal $\alpha$ analytically or experimentally.

We next consider the more general setting.
We evaluate how using a generative model improves performance as we vary (1) the number of samples $N$ from $p$ when creating $D_\texttt{train}$; (2) $\hat{p}(y)$ and (3) $p(y)$.
We compare the distributions with and without generated data for a specific example in \autoref{fig:bernoulli_single}.
For a more thorough experiment, for each choice of values, we resample $t(y)$ 1000 times and experimentally find the optimal $\alpha$.
We plot the optimal $\alpha$ as we vary these values in \autoref{fig:bernoulli_comprehensive}.
As can be seen, using generated is generally helpful (by the fact that $\alpha > 1$).
We can also see various properties.
First, as $N$ increases (e.g.~there is less distribution shift between $D_\texttt{train}$ and $p$), using generated data becomes less helpful as $\alpha$ goes to $0$.
Second, generated data is most useful when its distribution is more similar to the true distribution $p$, but generated data is helpful even in the face of some distribution shift between $p$ and $\hat{p}$.


\begin{comment}
% OLD VERSION
The generative model may go wrong in multiple ways, which we discuss in turn and how this impacts these choices.

\paragraph{Generative model is perfect.} In this case, the generative model always generates images with $\hat{p}(\vx | \va, y) = p_f(\vx | \va, y)$.
Provided we know $p_f(\va, y)$, we can simply set $\alpha = 0$ and sample $(\va, y) \sim p_f(\va, y), \vx \sim \hat{p}(\vx | \va,  y)$.

\paragraph{The generative model perturbs the label and attribute distribution.}
In this case, when we generate images, we sometimes generate images with a label different from the conditioning one.
We model this as a perturbation on the sampled label:
$\hat{p}(x|y, \va) \equiv p(x|\bar{y}, \bar{\va})p(\bar{y}, \bar{\va}|y, \va)$.
where the conditioning label and attributes are $(y, \va)$ and the true label and attributes of $\vx$ under an oracle is ($\bar{y}, \bar{\va}$).
Here we may sample images that are from the true distribution but have the wrong label.
We assume that for all samples in $D_t$, a model will perform perfectly. 
In the case where $D_t = D_f$, synthetic data will not help and we should set $\alpha=1$.
Therefore, we can only improve performance on samples present in $D_f$ but missing in $D_\texttt{train}$.

\noindent {\em Case 1: $p_\texttt{train}(y, \va) \ll p_f(y, \va) \frac{|D_f|}{|D_\texttt{train}|}$ for some $(y, \va)$:} 
In this case there are parts of the train set with only a handful of samples, which leads to poor generalisation.
We can write this as that there are many samples $(\vx, y, \va) \in D_f$ for which $p_\texttt{train}(\vx | y, \va) \approx 0$.
On these samples, the model would have to generalise, and we assume it generalises with an accuracy $a_\texttt{train}(y, \va)$. \olivia{Could say this is random but I don't agree with that as you should generalise to some extent, depending on how much data you have.}

The question is under what conditions will adding imperfect synthetic data improve performance. If the generative model has a non zero chance of generating such samples, then it will classify it accurately with probability $\hat{p}(\bar{y}=y|y, \va)$.
We sample $S$ synthetic examples under $\hat{p}$ and assume they are all valid images in $D_f$.
\olivia{Could make more 'proofy' by decomposing the expectation.}
Then, if we assume infinite capacity of the model, the accuracy will be the weighted average of the accuracy on the samples in $D_\texttt{train}$ and the generated samples.
So for synthetic samples to be helpful, we need the following condition to hold:
\begin{align}
    \frac{|D_\texttt{train}|^{y, \va}a_\texttt{train}(y, \va) + S \hat{p}(\bar{y}=y|y, \va)}{|D_\texttt{train}|^{y, \va} + S} &> a_\texttt{train}(y, \va) \\
    |D_\texttt{train}|^{y, \va} &= p_\texttt{train}(y, \va) |D_\texttt{train}|
\end{align}
This holds when $\hat{p}(\bar{y}=y|y, \va) > a_\texttt{train}(y, \va)$.
If we assume that $a_\texttt{train}(y, \va)$ will be similar to the proportion of missing data, we can write this as 
$\hat{p}(\bar{y}=y|y, \va) > \min(1, \frac{|D_\texttt{train}|^{y, \va} }{|D_f| p_f(y, \va)})$.
This gives the first area where synthetic data is useful: (1) generating data for low density regions improves performance in that region over training with real data alone.

\noindent {\em Case 2: $p_\texttt{train}(y, \va) = 0$ for some $(y, \va)$:}
In this case, the train set does not cover the full distribution and includes missing regions for which there are no samples.
Intuitively, provided we have a model with infinite capacity and a non zero probability of generating samples from these low data regions which will be correctly labelled with better than chance, then using synthetic data will improve performance.
Provided $\hat{p}(\bar{y}=y, \bar{\va}=\va|y, \va) > \frac{1}{\prod_i A_i Y}$ (i.e., better than random guess) and $\hat{p}(\vx | y, \va) > 0$, we will improve performance (assuming a model with infinite capacity) by including samples with label and attribute $(y, \va)$.
\olivia{Proof by decomposing expectation into regions and saying that we will now do better on these regions so overall we will do better.}
This gives the second area where synthetic data is useful: (2) datapoints which do not exist in $D_\texttt{train}$ but are correctly generated and with a better than chance probability given the correct label by the generative model.
\olivia{Could just fold this into the above tbh.}

\paragraph{Discussion.} Under these three scenarios, we expect that using synthetic samples should improve on using real data alone. Moreover, we find the following areas where using synthetic data will help.
First, if the synthetic data is able to generate data in low density regions that is correct with a probability better than the accuracy of the model in that region using \datasettrain alone.
Second, if the generative model is able to generate samples that do not exist in \datasettrain and classify them correctly with an accuracy better than chance.
\end{comment}

\subsection{A Bernoulli distribution over a labelled and hidden variable.}
The above case does not take into account that we can resample the dataset and use the conditioning variable of the generative model to make $D_\texttt{train}$ and $\hat{p}$ more similar to $p$.
However, in reality while we may be able to resample on a labelled variable, there will be many hidden attributes that are important for fairness and generalization.
As we do not have labels for these hidden attributes, we {\em cannot} resample over them to make the distribution more similar to $p$.

To explore this in a simplistic setting, we proceed as follows.
We assume we have two variables $a, y$ where $y$ is the label and $a$ some hidden attribute
which we want to be fair over (and generalise over). Again, they follow a Bernoulli distribution: $a \in \{0, 1\}$ and $y \in \{0, 1\}$.

We condition on the label and we can sample arbitrarily according to the label but this gives us a distribution over attributes conditioned on the label, which is fixed.  We can sample arbitrarily to create $\bar{t}(y)$ and $\bar{p}(y)$ (provided $t(y), \hat{p}(y) > 0$) but $\bar{t}(a|y) = t(a|y)$ and $\bar{p}(a|y) = \hat{p}(a|y)$ is fixed.
Again, the question is how to optimally combine $t(y, a)$ and  $\hat{p}(y, a)$.
So now 
\begin{align}
p'(y, a) &= t(a|y)\bar{t}(y) + \hat{p}(a|y)\bar{p}(y) \\
\sum_y \bar{t}(y) + \bar{p}(y) &= 1 
\end{align}

And again we want to minimize the KL divergence between these two distributions, which can be factorized into the sum of the KL divergence between the marginal distribution over $a$ and conditional distribution over $y$.
\begin{align}
KL(p'(a, y) || p(a, y)) = KL(p'(y) || p(y)) + KL(p'(a|y) || p(a|y))
\end{align}
This is hard to solve analytically but we can find the optimal distributions of $\bar{t}, \bar{q}$ for a given set of distributions experimentally.

\subsection{A high dimensional Gaussian Mixture Model (GMM)}
Here we demonstrate that additional unlabelled data can improve classification performance in a very simple setting.
We assume that points come from an underlying GMM where each mixture in the GMM correspond to a different class.
This GMM can have varying number of dimensions (the number of features) and components (the number of classes).
We demonstrate that using a generative model fit to some number of unlabelled points in combination with the labelled points can lead to improved performance of a trained classifier.

Given some number of labelled and unlabelled points, the aim is to train a classifier that performs well on a held out validation set.
We do this by fitting a GMM to the unlabelled points and then using the labelled points to determine what class each mode belongs to by minimizing the classification error on the labelled points.
We then combine the labelled points and some number of points sampled from the GMM to form the training set. 
This is used to train the classifier, which is evaluated on the validation set.

We plot the evolution of the GMM being fit to the unlabelled points as the number of unlabelled points varies next to the true, underlying GMM in \autoref{fig:gmm_visualisation}.
We plot the fitted GMM for varying numbers of unlabelled points.
With only 500 unlabelled points, the fitted GMM matches pretty closely the true distribution.

We then run the full pipeline including the downstream classifier for varying numbers of labelled (sampled points), generated points, components, and dimensions.
We always use 10K unsupervised points.
To create the GMM, we randomly sample means from the range $[0, 1]$ for each dimension and we create a full covariance metric under a normal distribution with a scale of $0.1$.
We plot the results in \autoref{fig:gmm_results}. 
In these three cases, we can see that using additional generated data improves performance.
However, this does not always happen if (1) the classifier already performs near perfectly using the labelled data or (2) there is an insufficient number of points or the mixtures overlap so much that fitting the generative model gives a poor estimate of the underlying distribution.

\begin{figure}[t]
\centering
\begin{overpic}[width=0.24\textwidth]{gmm/gt.pdf}
\put(35,95){\tiny True Distribution}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_1.pdf}
\put(32,95){\tiny 5 Unlabelled Points}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_4.pdf}
\put(27,95){\tiny 500 Unlabelled Points}
\end{overpic}
\begin{overpic}[width=0.24\textwidth]{gmm/frame_7.pdf}
\put(27,95){\tiny 5000 Unlabelled Points}
\end{overpic}
\caption{Visualising the fit GMM model for varying numbers of unlabelled points. Large points are labelled points, small points are unlabelled ones. Given only 500 unlabelled points, the fit distribution is similar to the true and with 5000 points, it matches the original. }
\label{fig:gmm_visualisation}
\end{figure}


\subsection{Discussion}
These toy experiments demonstrate that even in very simple settings, a generative model that complements in some way the data distribution can be used to create a new dataset that more closely mimics the underlying true distribution.
These two examples have shown in particular two scenarios where generative data can be especially helpful:
\begin{itemize}
    \item{\bf Missing regions.} Here the training data may not cover the full distribution. For example, if the training data has a label denoted by the random variable $y$ and attribute $a$ and there exists $y=y_c$, $a=a_c$ where there is no $x \in D_\texttt{train}$ such that $x \sim (y_c, a_c, ...)$.
    \item{\bf Low data regions.} Here there are only a few samples from parts of the distribution. If the generative model is able to capture this region then using additional samples from the generative model in this region should be helpful.
\end{itemize}

\section{Implementation}
\label{sec:implementation}

There are two main challenges. First, how to generate images with enough quality and diversity to be useful as additional synthetic data.
Second, how to combine real and synthetic data optimally for improved robustness and fairness.
We discuss these in turn.


\paragraph{The generator.}
We build on the diffusion model as popularized by \cite{Ho20}.
A diffusion model learns how to map images of gaussian noise to images from the distribution of training images.
Diffusion models have been leveraged to achieve state of the art, high quality results, with more diverse examples than with generative adversarial networks (GANs) \citep{Dhariwal21}.
The precise architecture we use is based on that of \cite{Dhariwal21} where we use a UNet with residual blocks and skip connections.

The architecture can be modified to allow for conditioning on auxiliary information \citep{Nichol21}, such as labels.
We use a one hot encoding of labels or labels and the sensitive attribute for conditioning.
When conditioning on both the label and sensitive attribute, we concatenate the one hot labels to form the final label.

\paragraph{Leveraging the unlabelled data.}
We can leverage ideas from classifier-free guidance to train a diffusion model with both labelled and unlabelled data.
Classifier-free guidance \citep{Ho21} trains both a conditional and unconditional diffusion model at the same time by randomly dropping some percentage of labels from the batch (by setting the label to $0$). 
At inference time, an image can be made more canonical by steering it away from the $0$-th label.
In our case, instead of randomly dropping labels, we treat the unlabelled data as dropped and set its label to the $0$-th label.
This allows us to train with both labelled and unlabelled data.
\olivia{Some insight here about how this modifies the sampling distribution.}

\paragraph{Super resolution?} Discuss how to work with larger image resolution sizes.

% \paragraph{Multiple instances?} Discuss how to generate multiple instances at once.

\paragraph{Combining real and synthetic data.}
The next step is to combine real and synthetic data.
Here there are two main considerations.
First, how to sample from the generative model and second how to trade-off between real and synthetic samples.
To sample from the generative model, we have to choose a distribution over the conditioning variable (the label or the label and auxiliary property).
We consider two distributions.
First, we can sample uniformly from the label or the joint distribution of label and auxiliary property.
However, this may harm overall performance.
Second, we can sample according to the label distribution in the training set but uniformly over the auxiliary property (if present).
This will increase diversity in the low data regions but not change the overall distribution of labels.
To trade-off between real and synthetic samples, we investigate combining batches of real and synthetic images with different ratios.
This effectively modifies the weight of the generative training in equation \ref{eq:finallikelihood}.


==> theoretical_motivation.tex <==
\section{Old write ups for theoretical motivation.}
\subsection{Theoretical Motivation 1}

To motivate why using generated samples should improve a classifier, we take inspiration from \cite{Lasserre07}. 
We first summarize their setup before describing how we utilise their framework.
We first assume we have a generative model which is specified as the product of the prior over classes $p(c|\pi)$ with the class conditional density $p(\vx|c,\lambda)$, where $\vtheta = \{ \pi, \lambda \}$.
This can be rewritten in terms of the likelihood $L_G(\vtheta)$.

\begin{align}
    p(\vx, c | \vtheta) = p(c | \pi) p(\vx | c, \lambda) \\
    L_G(\vtheta) = p(\rmX, \rmC, \vtheta) = p(\vtheta) \prod_{n=1}^N p(x_n, c_n | \vtheta)
\end{align}

However, as explained by \cite{Minka05} and \cite{Lasserre07}, we cannot simply use discriminative training, as that changes the model itself, not just the training method.
Instead \cite{Lasserre07} and \cite{Minka05} construct a new likelihood function $q$ that introduces a new set of parameters $\Tilde{\theta}$.
\begin{align}
    q(\vx, \vc| \vtheta, \Tilde{\vtheta}) &= p(\vc|\vx, \vtheta)p(\vx| \tilde{\vtheta}) \\
    p(\vx|\Tilde{\vtheta}) &= \sum_{\vc'}p(\vx, \vc'|\Tilde{\vtheta})
\end{align}

\cite{Lasserre07} then assume that the prior over parameters $p(\vtheta, \Tilde{\vtheta})$ factorizes:
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) = p(\vtheta)p(\Tilde{\vtheta})
\end{align}

This gives the following function to be maximised:
\begin{align}
    q(\rmX, \rmC, \vtheta, \Tilde{\vtheta}) &= p(\vtheta, \tilde{\vtheta}) \prod_{n=1}^{N} p(c_n | x_n, \vtheta)p(x_n|\Tilde{\vtheta}) \\
    &= \left[ p(\vtheta) \prod_{n=1}^{N} p(c_n| x_n, \vtheta) \right]  \left[ p(\Tilde{\vtheta}) \prod_{n=1}^{N} p(x_n | \Tilde{\vtheta}) \right]
\end{align}

\paragraph{An equality prior.}
If the parameters are independent then this is simply discriminative training.
The question is how to construct the prior over $\vtheta, \Tilde{\vtheta}$ when the parameters $\vtheta, \Tilde{\vtheta}$ are not independent.
\cite{Lasserre07} consider an equality prior.
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) = p(\vtheta)\delta(\vtheta - \Tilde{\vtheta})
\end{align}
If $\Tilde{\vtheta} = \vtheta$ then we can see that the joint distribution of $q$ simplifies to the original generative model.
This can be loosened by considering priors from a laplace distribution to give a smooth transition between pure discriminative/generative training.
Which set up is optimal depends whether the data is truly from the generative model.
If it is, then the hard constraint is preferable, allowing for the use of the additional data.
If it is not, then we can still improve on discriminative training depending on how the generative model is constructed and the additional, unlabelled data improves model performance. This requires experimental investigation in practice.

\paragraph{Forcing consistency.}
In our case, it is not simple to impose a constraint directly on the model parameters, as the models are trained separately with different model parameters. Instead, we aim to achieve the coupling of the generative and discriminative models by imposing a consistency constraint in the prior.
Now, instead of in \cite{Lasserre07}, we do not consider an equality prior but instead a prior that predictions must be consistent between the two models. 

 If the generator generates an image, label pair $(x'_k, c'_k)$ with image $x'_k$ and label $c'_k$ then the discriminative model should predict that sample to have the same label.
We have the following where $\rmX'$ denotes the $N_s$ sampled images and $\rmC'$ the sampled classes and we assume $\vtheta, \Tilde{\vtheta}$ are independent variables. \olivia{I don't think this is right: should be integrating over $x'_k, {c'_k}$ which would give a sum. All this should be checked by Taylan.}:
\begin{align}
    p(\vtheta, \Tilde{\vtheta}) &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC' | \vtheta, \Tilde{\vtheta})} \\
     &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC' |
    \vtheta) p(\rmX', \rmC' | \Tilde{\vtheta})} \\
     &= \frac{p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC')}{p(\rmX', \rmC') p(\rmX', \rmC' | \Tilde{\vtheta})} \\
    p(\vtheta, \Tilde{\vtheta}, \rmX', \rmC') &= p(\vtheta, \Tilde{\vtheta} | \rmX', \rmC') p(\rmX', \rmC') \\
    &= p(\vtheta |\rmX', \rmC') p(\Tilde{\vtheta} | \rmX', \rmC') p(\rmX', \rmC') \\
    &= \frac{p(\vtheta)p(\rmC' | \rmX', \vtheta)}{p(\rmC' | \rmX')} p(\rmX', \rmC' | \Tilde{\vtheta}) p(\Tilde{\vtheta}) \\
    p(\vtheta, \Tilde{\vtheta}) &= \frac{p(\vtheta)p(\rmC' | \rmX', \vtheta)}{p(\rmC' | \rmX')^2 p(\rmX')} p(\Tilde{\vtheta}) \\
\end{align}

Now we assume these samples are independent to get a new joint distribution:
\begin{align}
    q(\rmX, \rmC, \vtheta, \Tilde{\vtheta}) = \left[ \prod_{n=1}^{S} \frac{p(c'_n|x'_n, \vtheta)}{p(c'_n|x'_n)^2 p(x'_n)} \right] \left[ p(\vtheta) \prod_{n=1}^{N} p(c_n| x_n, \vtheta) \right]  \left[ p(\Tilde{\vtheta}) \prod_{n=1}^{N} p(x_n | \Tilde{\vtheta}) \right]
    \label{eq:finallikelihood}
\end{align}

\paragraph{Special case: the generative model subsumes the training set.}
If the generative model subsumes the training set and is perfect than $p(c'_n | x'_n) = 1, p(x'_n) = 1$ and we can see that optimizing the discriminative model over the generated samples is sufficient to optimize it over the real samples. 

If it is not, then optimizing the discriminative model over the generated samples amounts to having a regularizer with a weight $\lambda$ that is controlled by the coefficient $\frac{1}{\prod_{n=1}^{N_s} p(c'_n|x'_n)^2 p(x'_n)}$. 
As this quantity is unknown, we can sweep over this value experimentally (from $1$ to $\infty$) to find the optimal trade off for the discriminative model between generated and real examples.
